Scalable Multivariate Fronthaul Quantization for Cell-Free Massive MIMO

The conventional approach to the fronthaul design for cell-free massive MIMO system follows the compress-and-precode (CP) paradigm. Accordingly, encoded bits and precoding coefficients are shared by the distributed unit (DU) on the fronthaul links, and precoding takes place at the radio units (RUs). Previous theoretical work has shown that CP can be potentially improved by a significant margin by precode-and-compress (PC) methods, in which all baseband processing is carried out at the DU, which compresses the precoded signals for transmission on the fronthaul links. The theoretical performance gain of PC methods are particularly pronounced when the DU implements multivariate quantization (MQ), applying joint quantization across the signals for all the RUs. However, existing solutions for MQ are characterized by a computational complexity that grows exponentially with the sum-fronthaul capacity from the DU to all RUs. This work sets out to design scalable MQ strategies for PC-based cell-free massive MIMO systems. For the low-fronthaul capacity regime, we present alpha-parallel MQ (alpha-PMQ), whose complexity is exponential only in the fronthaul capacity towards an individual RU, while performing close to full MQ. alpha-PMQ tailors MQ to the topology of the network by allowing for parallel local quantization steps for RUs that do not interfere too much with each other. For the high-fronthaul capacity regime, we then introduce neural MQ, which replaces the exhaustive search in MQ with gradient-based updates for a neural-network-based decoder, attaining a complexity that grows linearly with the sum-fronthaul capacity. Numerical results demonstrate that the proposed scalable MQ strategies outperform CP for both the low and high-fronthaul capacity regimes at the cost of increased computational complexity at the DU (but not at the RUs).

==> Sections/1_Intro.tex <==
%However, in order to support ultra-large-scale MIMO at the single base station (BS), a complicated chip specification is needed to handle all the functionalities required for MIMO data transmission. To this end, functional split \cite{checko2014cloud} has been proposed as a key solution.

%splits the burden of BS t



\section{Introduction}
\label{sec:intro}
One of the most effective ways of enhancing the capacity of wireless link is to increase the number of antennas \cite{tse2005fundamentals}. In 5G systems, this is facilitated by the disaggregation of the functionalities of a base station (BS) between a central unit (CU) and multiple distributed units (DUs), which are connected to the CU via fronthaul links. As illustrated in Fig.~\ref{fig:system_model_general}-(\emph{i}), the collection of all DUs has the potential of acting as a single, distributed, ultra-large-scale MIMO system. 





As prescribed by enhanced common public radio interface (eCPRI), different funtional splits between CU and DUs are possible. A first, common approach is to evaluate  the precoding matrix at the CU, which is transmitted to every DU along with all the information bits to be encoded on the fronthaul. The fronthaul overhead of this approach scales linearly with the data sum-rate and  hence also with the number of users. Furthermore, all DUs need to apply channel encoding and precoding for all users. To mitigate these problems, an alternative functional split has been introduced  in which the CU applies coding and precoding, then transmits to each DU the respective complex baseband signals \cite{park2013joint, lee2016multivariate}. This way, as suggested by the theoretical results in \cite{park2013joint,sanderovich2009uplink, simeone2012cooperative}, the fronthaul capacity does not need to scale as quickly with the sum-rate and computational complexity at the DUs is reduced to decompression. 


While the functional split has the potential to effectively lessen the fronthaul capacity and the computational burden of the DUs, the theoretical results in \cite{park2013joint} assume complex forms of baseband compression at the CU, whose practical implementation is unclear. The standard design considers scalar quantization or, more generally, point-to-point (per-DU) compression techniques. Recently, motivated by the network-information theoretic results, a form of \emph{multivariate quantization} that compresses all baseband  signals jointly has been proposed in \cite{lee2016multivariate}. 

Reference  \cite{lee2016multivariate} proposed a \emph{data-driven} algorithm for multivariate quantization that was shown to outperform existing point-to-point compression techniques. The algorithm in \cite{lee2016multivariate} suffers from exponentially growing computational complexity in the fronthaul sum-rate, and it is limited to the optimization of a performance criterion that does not directly relate to achievable rates. In this project, we aim at addressing these shortcomings of the state of the art by designing a multivariate quantizer with complexity growing linearly in the fronthaul sum-rate via \emph{graph-based quantizer} that can address any (non-convex, non-linear) utility function of interest. 

%Detailed limitations of the state-of-the-art multivariate quantization \cite{lee2016multivariate} can be found in Sec.~\ref{sec:sota}.

\begin{figure}
 \begin{center}\includegraphics[scale=0.18]{Figs/system_model_general_original.pdf}
   \end{center}
   \caption{Distributed antenna architecture considered in this project consisting of $N$ UEs, $M$ DUs and a CU. All baseband processing is done at the CU, which carries out compression of the baseband signals via multivariate compression}
   \label{fig:system_model_general}
\end{figure}


The proposed algorithm builds on a theoretical insight presented in \cite{park2013joint}. This paper shows that, in the limit of long quantization blocks, one can without loss of optimality quantize signals for different DUs in a sequential way. Based on this insight, we view the problem of multivariate quantization as the design of an autoencoder architecture with a graph-based encoder, a distributed decoder, and discrete bottleneck variables between encoder and decoder. The encoder leverages graph neural networks \cite{velivckovic2023everything}, which mimic and generalize the sequential architecture suggested by the theory. Furthermore,  adaptation based on CSI is ensured via hypernetworks \cite{ha2016hypernetworks}. Overall, the proposed system aims at ensuring both scalability and low-complexity for the joint design of precoding and compression. 

Graph-based approaches have been applied to communication systems to ensure scalability via modular structure. This has been proved to be useful in various applications, including power control \cite{nikoloska2022modular} and precoding matrix design \cite{shen2022graph, zhao2022understanding}. Hypernetworks constitute a special form of meta-learning that can facilitate adaptation to the channel conditions. This idea has also shown remarkable success in wireless communications, especially for providing coherent solutions to time-varying channels, e.g., for precoding design \cite{liu2022learning} and MIMO detection \cite{goutay2020deep}. 

==> Sections/3_b_EI_for_multi_antennas.tex <==
\section{Effective Interference}

In this section, we generalize the EI \eqref{eq:EI_def} and the effective SINR in \eqref{eq:average_sinr_sota} by taking into account for presence of  multi-antenna DUs and  multi-antenna UEs, as well as channel estimation noise at the receiver side. 

\subsection{Effective SINR and Effective Interference}
As defined in \eqref{eq:rx_basic}, the $N_n^\text{rx} \times 1$ received signal vector $y_n$ at the UE $n$ is given by
\begin{align}
    \label{eq:rx_multi}
    y_n &=  H_n \hat{x} + z_n \nonumber \\&
    = H_n(W_{n}s_n) +  H_n(\hat{x}-W_ns_n) + z_n.
\end{align}
In \eqref{eq:rx_multi}, we have distinguished between the contribution of the useful signal, $H_n(W_n s_n)$, of the quantization noise, $H_n(\hat{x}-W_ns_n) $, and of the channel noise, $z_n$.

Accordingly, the average effective SINR for UE $n$ is defined as the ratio \begin{align}
    \label{eq:average_sinr_multi_antenna}
    &\text{SINR}_n \\&= \frac{\mathbbm{E}_{H}\big[||H_n W_{n}||^2\big]}{N_n^\text{rx}\sigma^2 +\mathbbm{E}_{H,s}\bigg[ \Big|\Big|H_n \Big(\hat{x}-x + \sum_{n' \neq n}W_{n'}s_{n'}\Big)\Big|\Big|^2\bigg]},\nonumber
\end{align}
where the numerator is the power of the useful signal and the denominator is the power of the overall disturbance caused by quantization noise and channel noise. From \eqref{eq:average_sinr_multi_antenna}, the EI for UE $n$ is defined equivalently as {\color{blue}  \begin{align}
\label{eq:EI_multi_antenna}
\text{EI}_n (\hat{x}) = \text{tr}\big( H_n K(\hat{x})H_n^\dagger \big),
\end{align}
where 
\begin{align}
    K(\hat{x})=\mathbb{E}_{s}\big[(\hat{x}-W_ns_n)(\hat{x}^\dagger - s_n^\dagger W_n^\dagger)\big]
\end{align}
is the covariance matrix of the effective interference.  Note that \eqref{eq:average_sinr_multi_antenna} and \eqref{eq:EI_multi_antenna} recover \eqref{eq:average_sinr_sota} and \eqref{eq:EI_def}, respectively, for $N_m^\text{tx}=N_n^\text{rx}=L_n=1$.

Treating noise and interference as worst-case Gaussian noise, the sum-rate can be computed as \cite{tse2005fundamentals}
\begin{align}
\label{eq:multi_antenna_sum_rate}
    &\sum_{n=1}^N\log_2 \left(\frac{ \det \Big( \mathbb{E}_{H,s} [y_n y_n^\dagger] \Big) }{\det\Big(\sigma^2 I + \mathbb{E}_{H,s}\big[H_n K(\hat{x}) H_n^\dagger \big] \Big)}\right) \\\nonumber 
    &= \sum_{n=1}^N\log_2 \left(\frac{ \det \Big( \mathbb{E}_{H,s} [ H_n\hat{x}\hat{x}^\dagger H_n^\dagger  ] + \sigma^2 I \Big) }{\det\Big(\sigma^2 I + \mathbb{E}_{H,s}\big[H_n K(\hat{x}) H_n^\dagger \big] \Big)}\right) 
    \\\nonumber&\approx \sum_{n=1}^N\log_2 \left(\frac{ \det \Big(\mathbb{E}_{H,s} \big[H_n W_n W_n^\dagger H_n^\dagger + \sigma^2 I + \mathbb{E}_{H,s}\big[H_n  K(\hat{x}) H_n^\dagger\big]   \big] \Big) }{\det\Big(\sigma^2 I + \mathbb{E}_{H,s}\big[H_n K(\hat{x}) H_n^\dagger \big] \Big)}\right), 
\end{align}
With single-antenna UEs, the expression \eqref{eq:multi_antenna_sum_rate} reduces to $\sum_{n=1}^N\log_2(1+\text{SINR}_n)$ bits/s/Hz \cite{lee2016multivariate}. 


% %Evaluation of the sum-rate of the UEs can be computed as
% \begin{align}
%     \sum_{n=1}^N\log_2 \frac{ \det \Big(\sigma^2 I + \mathbb{E}_{H,s}\big[H_n  K_{\hat{x}_n} H_n^\dagger\big]  + \mathbb{E}_{H,s} \big[H_n K_{x_n} H_n^\dagger \big] \Big) }{\det\Big(\sigma^2 I + \mathbb{E}_{H,s}\big[H_n K_{\hat{x}_n} H_n^\dagger \big] \Big)}, \label{eq:multi_antenna_sum_rate}
% \end{align}
% with $K_{\hat{x}_n} = (\hat{x}-W_ns_n)(\hat{x}^\dagger - s_n^\dagger W_n^\dagger)$ and
% $K_{x_n} = W_n  W_n^\dagger $. With single-antenna UEs, the expression \eqref{eq:multi_antenna_sum_rate} becomes $\sum_{n=1}^N\log_2(1+\text{SINR}_n)$ bits/s/Hz \cite{lee2016multivariate}. 

}





\subsection{Effective SINR with Channel Estimation Noise}
The effective SINR \eqref{eq:average_sinr_multi_antenna} is a suitable performance measure when one assumes that the UEs have a sufficiently accurate estimate of the respective channels. In practice, each UE $n$ needs to estimate its respective channel, i.e., $N_n^\text{rx}\times L_n$ channel matrix after precoding which we denote as $G_n=H_nW_n$,  using $N_p \geq 1$ pilots. Here, we generalize the expressions of SINR \eqref{eq:average_sinr_multi_antenna} and EI \eqref{eq:EI_multi_antenna} to account for channel estimation error. 


Denoting as $s^\text{p}_{i,n}$ the $i$-th pilot vector of size $L_n$ intended for UE $n$, CU precodes the $L\times 1$  vector $s_i^\text{p}=[(s_{i,1}^\text{p})^\top,...,(s_{i,N}^\text{p})^\top]^\top$ via the precoding matrix $W$ as 
\begin{align}
    x_i^\text{p} = W s_i^\text{p}
\end{align}
for $i=1,...,N_p$. The precoded pilots $x_i^\text{p}$ are quantized as for the data symbols, producing the quantized signals $\hat{x}^{\text{p}}_i=Q(x_i^\text{p})$.

In a manner analogous to \eqref{eq:rx_multi}, the signal received by UE $n$ can be written as
\begin{align}
    \label{eq:rx_single_pilots}
    y_{i,n}^\text{p} &=  H_n \hat{x}_i^\text{p} + z_{i,n} \nonumber \\&
    = H_n(W_{n}s_{i,n}^\text{p}) +  H_n(\hat{x}_i^\text{p}-W_ns_{i,n}^\text{p}) + z_{i,n}.
\end{align}
Denoting the collection of $N_p$ pilot vectors as the $L \times N_p$ matrix $S^\text{p} = [s^\text{p}_1,...,s^\text{p}_{N_p}]$, and as $S_n^\text{p}=[s_{1,n}^\text{p},...,s_{N_p,n}^\text{p}]$ the $L_n \times N_p$ matrix  of pilots for the UE $n$, the corresponding received signals \eqref{eq:rx_single_pilots} for all pilots symbols can be written as the $N_n^\text{rx} \times N_p$ matrix
\begin{align}
    \label{eq:rx_multi_pilots}
    Y_n^\text{p} &=  H_n \hat{X}^\text{p} + Z_n \nonumber \\&
    = H_n(W_{n}S_n^\text{p}) +  H_n(\hat{X}^\text{p}-W_n S_n^\text{p}) + Z_n,
\end{align}
where we have defined $\hat{X}^\text{p}=[\hat{x}_1^\text{p},...,\hat{x}_{N_p}^\text{p}]$ as the $N^\text{tx} \times N_p$ matrix of quantized pilot vectors and $Z_n = [z_{1,n}, ..., z_{N_p,n}]$  as the $N_n^\text{rx}\times N_p$ matrix of noise vectors for UE $n$. 





% $N_n^\text{rx} \times l_n$ channel matrix \emph{after} precoding, i.e., $H_n W_n$, using $N_D$ pilots in which the $i$-th pilot is defined as $L\times 1$ vector $d_i=[d_{i,1}^T, ..., d_{i,N}^T]^T$ (cf. definition of $s$ in Sec.~\ref{sec:sys_model}) that satisfies $\mathbb{E}[d_i d_i^\dagger] = I_{L}$ for all $i=1,...,N_D$. Accordingly, we define the collection of the pilots $D=[d_1,...,d_{N_D}]$ as the \emph{pilot matrix}, and its submatrix that corresponds to UE $n$ as $D_n$, i.e., matrix that takes rows from $(\sum_{n'=1}^{n-1} l_{n'}+1)$-th  to $(\sum_{n'=1}^{n} l_{n'})$-th of $D$. We further assume that the submatrix $D_n$ is a fat matrix for all $n=1,...,N$, i.e., $N_D \geq \max_n \{l_n\}$.

% From \eqref{eq:rx_multi}, by taking $d_i$ in lieu of $s$, we can get $i$-th pilot data which will be collectively used to estimate the channel matrix for each UE $n$. First let us denote the corresponding received pilot signal as $y_{i,n}^\text{p}$, the received noise vector as $z_{i,n}^\text{p}$, and the entire transmit vector as $\hat{x}_i^\text{p}$. Furthermore, we denote their corresponding $N_D$ collections  as $Y_n^\text{p}=[y_{1,n}^\text{p},...,y_{N_D,n}^\text{p}]$, $Z_n^\text{p}=[z_{1,n}^\text{p},...,z_{N_D,n}^\text{p}]$, and $\hat{X}^\text{p} = [\hat{x}_{1}^\text{p},...,\hat{x}_{N_D}^\text{p}]$. 

 
% \begin{figure}[h]
%     \begin{center}\includegraphics[scale=0.28]{Figs/tree_index.pdf}
%       \end{center}
%       \caption{...}
%       \label{fig:tree_indexing}
%    \end{figure}


Adopting a maximum likelihood estimator, the  channel for each UE $n$ can be estimated from the received $N_p$ pilots as  
\begin{align} \label{eq:hat_H_n}
    \hat{G}_{n} &= Y_n^\text{p} {(S_n^\text{p})}^{-1} \nonumber \\&
    = \underbrace{H_n W_{n}}_{ \substack{= \text{ respective channel} \\ \substack{ \text{ for UE $n$}, G_n}}} + \underbrace{H_n \hat{X}^\text{p} {(S_n^\text{p})}^{-1} - H_n W_n  + Z_n {(S_n^\text{p})}^{-1}}_{=\text{ channel estimation error, $E_n$}},
\end{align}
where we denoted ${(S_n^\text{p})}^{-1}$ as the  Moore–Penrose right pseudoinverse of the (fat) matrix $S_n^\text{p}$. Note that, as the number of pilots $N_p$ increases, the last term in the channel estimation error $E_n$, $Z_n{(S_n^\text{p})}^{-1}$, becomes vanishingly small; while, when the fronthaul capacity increases, the first and second terms of the error $E_n$ tend to cancel each other out since $\hat{X}^\text{p}$ becomes increasingly close to $W_nS_n^\text{p}$. 


Now, we can rewrite \eqref{eq:rx_multi} in terms of the estimate $\hat{G}_n$ as 
\begin{align}
    \label{eq:rx_multi_noisy_ch_est}
    y_n 
    =\hat{G}_n s_n +  H_n (\hat{x}- W_ns_n) - E_n s_n + z_n.
\end{align}
Therefore, by treating channel estimation error as worst-case Gaussian noise (see, e.g., \cite{hassibi2003much, yoo2006capacity}), the average effective SINR for UE $n$ can be expressed  as
\begin{align}
    \label{eq:average_sinr_multi_est_noise}
    &\text{SINR}_n = \frac{ \mathbbm{E}_{H}\big[|| \hat{G}_n ||^2\big]}{N_n^\text{rx}\sigma^2 +\mathbb{E}_{H,s}\big[\text{EI}_n(\hat{x})\big] + \mathbb{E}_{H,Z_n}\big[||E_n||^2\big]  }.
\end{align}

The average effective SINR \eqref{eq:average_sinr_multi_est_noise} generalizes the expressions in \eqref{eq:average_sinr_sota} and \eqref{eq:average_sinr_multi_antenna} by accounting for both multi-antenna DUs and UEs and for the channel estimation error. %This will be used to evaluate the sum-rate in the presence of channel estimation noise, i.e., 
{\color{blue} Accordingly, as in \eqref{eq:multi_antenna_sum_rate}, sum-rate in the presence of channel estimation noise can be expressed as $\sum_{n=1}^N \log_2 r_n$ with 
\begin{align}
    &r_n =\nonumber\\&\frac{ \det \Big(   \sigma^2 I + \mathbb{E}_{H,s,Z_n}\big[H_n K_{\hat{x}_n} H_n^\dagger - A_n\big]  + \mathbb{E}_{H,Z_n}[E_n E_n^\dagger] + \mathbb{E}_{H}[\hat{G}_n\hat{G}_n^\dagger]  \Big) }{\det\Big(\sigma^2 I + \mathbb{E}_{H,s,Z_n}\big[H_n K_{\hat{x}_n} H_n^\dagger - A_n\big]  + \mathbb{E}_{H,Z_n}[E_n E_n^\dagger]   \Big)}, \label{eq:multi_antenna_sum_rate_ch_est}
\end{align}
given $A_n = 2 \cdot \text{Re}\big(H_n(\hat{x}-W_ns_n)s_n^\dagger E_n^\dagger\big) $. With single-antenna UEs, the expression \eqref{eq:multi_antenna_sum_rate_ch_est} becomes $\sum_{n=1}^N\log_2(1+\text{SINR}_n)$ bits/s/Hz \cite{lee2016multivariate} when assuming $\mathbb{E}[A_n]=0$ -- worst-case Gaussian noise.}

% Hence, from
% \begin{align}
%     \mathbb{E}_{z_n}[||e_n||^2] &= \mathbb{E}[ \text{tr}(e_n e_n^\dagger) ] 
%     \nonumber\\& = \mathbb{E}\bigg[ l_n||H_n \hat{x}^\text{p}||^2 + ||H_n W_n||^2 + \frac{l_n}{P}N_n^\text{rx} \bigg],
% \end{align}
% we define average effective SINR for UE $n$ that takes into account for the channel estimation noise as
% \begin{align}
%     \label{eq:average_sinr_multi_est_noise}
%     &\text{SINR}_n \nonumber\\ = &\frac{P \mathbbm{E}_{H}\big[||H_n W_{H,n}||^2\big]}{N_n^\text{rx}\sigma^2 +P \mathbb{E}_{H,s}\big[\text{EI}_n(\hat{x}) +  l_n||H_n \hat{x}||^2 + ||H_n W_n||^2\big] + l_n N_n^\text{rx}  },
% \end{align}


% Accordingly, we define average effective SINR for UE $n$ as
% \begin{align}
%     \label{eq:average_sinr_sota}
%     \text{SINR}_n = \frac{P \mathbbm{E}_{H}\big[||H_n W_{H,n}||^2\big]}{N_n^\text{rx}\sigma^2 +P\mathbbm{E}_{H,s}\big[ ||H_n (\hat{x}-x + \sum_{n' \neq n}W_{H,n'}s_{n'})||^2]},
% \end{align}
% using the Frobenius norm operator $||\cdot||$. 












==> Sections/3_b_EI_tmp.tex <==
{\color{blue}
    \section{Computational Computational Analysis} \label{sec:detailed_comp_complexity}
In this section, we compare the computational complexity of CP and PC in terms of number of floating point operations (flops). Since CP and PC have different functional split as described throughout the paper, we will make the comparison at the DU and RU side separately. In order to provide explicit flops formula, we first describe the simple  MMSE precoding design adopted in this work, which can again be justified in cell-free massive MIMO system in a manner similar to the localized receiver design (\ref{eq:simpler_MMSE_receiver_beamforming}).


\subsection{MMSE Precoding Design}\label{subsec:mmse_precoding}
Given the $N^\text{rx} \times N^\text{tx}$ full channel matrix $H = [H_1^\dagger,...,H_N^\dagger]^\dagger$, we first reduce the dimension of row space of $H_n$ from $N_n^\text{rx}$ to $L_n$ by projecting $H_n$ to the reduced eigenspace of $H_n H_n^\dagger$ constructed by $L_n$ eigenvectors with $L_n$-largest singular values, i.e., obtain dimension-reduced matrix $\tilde{H}_n$ as 
\begin{align}
    \tilde{H}_n = U_{:, 1:L_n}^\dagger H_n, 
\end{align}
denoting as $U_{:, 1:L_n}$ the collection of the first $L_n$ columns of $U_n$ given $H_n = U_n \Sigma_n V_n^\dagger$. We assume that singular values in $\Sigma_n$ are sorted in a descending order. Then we can obtain the standard MMSE precoding matrix $W$ given $\tilde{H} = [\tilde{H}_1^\dagger, ..., \tilde{H}_N^\dagger]^\dagger$ and a power scaling factor $r_m$ for RU $m$ as
\begin{align}
    W = \text{diag}(r_1,...,r_M) \cdot \tilde{H}^\dagger (\tilde{H}\tilde{H}^\dagger + \xi I)^{-1},
\end{align}
given the regularization factor $\xi = N^\text{rx}/\sum_{m=1}^M P_m$ \cite{schmidt2008minimum}. Denoting as $\tilde{W} = \tilde{H}^\dagger (\tilde{H}\tilde{H}^\dagger + \xi I)^{-1} $ the unnormalized precoding matrix, the power scaling factor $r_m$ can be obtained as 
\begin{align}
    r_m = \sqrt{\frac{P_m}{\text{tr}(\tilde{W}_m^\dagger \tilde{W}_m)}}, 
\end{align}
with  $\tilde{W}_m$ the unnormalized precoding matrix associated to RU $m$. Corresponding computational complexity analysis for the precoding design can be found in Table~\ref{table:tab_comp_comp_DU} (row $1$--$6$) in Appendix~\ref{app:comp_analysis}.



%with $N_n^\text{rx}\times N^\text{tx}$ per-UE channel matrix $H_n$ for UE $n$,

% \subsection{MMSE Precoding Design}\label{subsec:mmse_precoding}
% Given the $N^\text{rx} \times N^\text{tx}$ full channel matrix $H = [H_1^\dagger,...,H_N^\dagger]^\dagger$, we first reduce the dimension of row space of $H_n$ from $N_n^\text{rx}$ to $L_n$ by projecting $H_n$ to the reduced eigenspace of $H_n H_n^\dagger$ constructed by $L_n$ eigenvectors with $L_n$-largest singular values, i.e., obtain dimension-reduced matrix $\tilde{H}_n$ as 
% \begin{align}
%     \tilde{H}_n = U_{:, 1:L_n}^\dagger H_n, 
% \end{align}
% denoting as $U_{:, 1:L_n}$ the collection of the first $L_n$ columns of $U_n$ given $H_n = U_n \Sigma_n V_n^\dagger$. We assume that singular values in $\Sigma_n$ are sorted in a descending order. Then we can obtain standard MMSE precoding matrix $W$ given $\tilde{H} = [\tilde{H}_1^\dagger, ..., \tilde{H}_N^\dagger]^\dagger$ and a power scaling factor $r_m$ for RU $m$ as
% \begin{align}
%     W = \text{diag}(r_1,...,r_M) \cdot \tilde{H}^\dagger (\tilde{H}\tilde{H}^\dagger + \xi I)^{-1},
% \end{align}
% given the regularization factor $\xi = N^\text{rx}/\sum_{m=1}^M P_m$ \cite{schmidt2008minimum}. Denoting as $\tilde{W} = \tilde{H}^\dagger (\tilde{H}\tilde{H}^\dagger + \xi I)^{-1} $ the unnormalized precoding matrix, the power scaling factor $r_m$ can be obtained as 
% \begin{align}
%     r_m = \sqrt{\frac{P_m}{\text{tr}(\tilde{W}_m^\dagger \tilde{W}_m)}}, 
% \end{align}
% with  $\tilde{W}_m$ the unnormalized precoding matrix associated to RU $m$. Corresponding computational complexity analysis for the precoding design can be found in Table~\ref{table:tab_comp_comp_DU} (row $1$--$6$).

\subsection{Computational Complexity Comparison}
In this subsection, we revisit the overall process of both CP and PC at DU and RU side to clarify the  associated computational complexities. We assume $D_m=D$ and $K_m=1$  for all $m=1,...,M$ to avoid clutter. On the one hand, at DU side, CP needs to carry out precoding design, while PC needs additional quantization process as shown in row $7$ of Table~\ref{table:tab_comp_comp_DU} (Appendix~\ref{app:comp_analysis}}). On the other hand, at RU side, CP needs to apply precoding matrix $W$ to the symbol vector $s$, i.e., $W s$ (row $1$ of Table~\ref{table:tab_comp_comp_RU}, Appendix~\ref{app:comp_analysis}), while for PC, it requires single inference of the neural network (row $2$ of Table~\ref{table:tab_comp_comp_RU}, Appendix~\ref{app:comp_analysis}). In the tables, we have assumed that complex multiplication requires $3$ times more flops as compared to real multiplication.  

% \begin{figure}[h]
%   \begin{center}\includegraphics[scale=0.3]{Figs/huawei_computation.pdf}
%     \end{center}
%     \caption{Condition of total number of streams  to ensure lower computational complexity of PC as compared to CP: (a) Two regions are shown where the green region is the case in which the complexity of CP is higher than PC, i.e.,  $L > {2D_m}/{3} + {B_m\cdot D_m}/{3N_m^{tx}}$; while the red region corresponds to higher complexity of PC than CP, i.e.,  $L < {2D_m}/{3} + {B_m\cdot D_m}/{3N_m^{tx}}$. We assume $D_m=B_m$ here. (b) Different boundaries can be obtained for different numbers of hidden neurons $D_m = \{B_m/6, B_m/3, B_m/2, B_m\})$. {\color{red}check $D_m$} }
%     \label{fig:computaion_comp_illust}
%  \end{figure}
 
At the first glance, PC may seem to require higher computational complexity at both DU and RU side as compared to CP. However,  depending on the total number $L$ of streams, at the RU side,  computational complexity of CP can be higher than that of PC, since PC is independent with the size of the signal vector $s$ from its inherent \emph{precoding-then-compress} design. For instance, from Table~\ref{table:tab_comp_comp_RU}, it can be easily checked that for $L > {2D}/{3} + {B_m\cdot D}/{3N^{tx}}$, computational complexity of CP is higher than that of PC. 



% We make this point clear in  Fig.~\ref{fig:computaion_comp_illust}. First, from Table~\ref{table:tab_comp_comp_RU}, it can be easily checked that for $L > {2D}/{3} + {B_m\cdot D}/{3N_m^{tx}}$, computational complexity of CP is higher than that of PC. Fig.~\ref{fig:computaion_comp_illust}(a) depicts this corresponding boundary condition under $D_m=B_m$ with $N_m^\text{tx}=16$. Furthermore, since such boundary is dependent on the size of the neural network, we then plot different boundaries by varying the size of the neural network in Fig.~\ref{fig:computaion_comp_illust}(b). As shown in the figure, by adopting smaller neural network with less hidden neurons $D_m$, PC can  further decrease the computational complexity. Note that quantization of the neural network parameters \cite{zhou2017incremental, przewlocka2022power, gholami2022survey} can also significantly reduce the computational complexity of neural-MQ. 

% Form  Fig.~\ref{fig:computaion_comp_illust}, and from the description of the fronthaul constraint of CP (\ref{eq:CP_constraint}), it is  clear that PC via neural-MQ can significantly reduce both the fronthaul overhead and the computational complexity at the RU side especially when the total number $L$ of streams are large -- the case where the cell-free MIMO system typically encounters \cite{ngo2024ultra}. In the remaining parts of the paper, we will experimentally validate this aspect, with total computational complexity comparison at both the DU and RU side for PC and CP is briefly discussed at the last part of this work {\color{red} (Fig.~\ref{fig:})}. In general, neural-MQ has higher computational complexity than CP at the DU side due to the multiple number $I$ of GD steps in (\ref{eq:GD_for_neural_MQ}). }

%Reducing the number of GD steps possibly aided by the model-based learning \cite{shlezinger2022model} or even via  meta-learned transformers \cite{jain2024mnemosyne} would be an interesting future work direction. }


% Now the last remaining question is how much additional computational complexity burden is required by PC as compared to CP at the DU side. As shown in Table~\ref{table:tab_comp_comp_DU}, PC complexity linearly scales with the number of GD steps $I$ hence it is important to reduce $I$ when one wants to decrease the complexity at the DU side. In the next section, we describe \emph{sequential neural-MQ} which outperforms neural-MQ in the presence of limited number of GD iterations $I$. 





% Now let us denote as $C_W$ the computational complexity required by precoding design as well as the channel coding, and also further denoting as $C^\text{DU}_\text{CP}$ and $C^\text{RU}_\text{CP}$  the computational complexity of CP at DU and RU, respectively, and finally denote as $C^\text{DU}_\text{PC}$ and $C^\text{RU}_\text{PC}$ the computational complexity of PC at DU and RU, respectively. 







% Table~\ref{table:tab_comp_comp_DU} and Table~\ref{table:tab_comp_comp_RU} that also encompass the complexities of  both CP and the proposed neural-MQ.






% \section{Sequential Neural Multivariate Quantization} \label{sec:sequential_neural_MQ}
% We first recall that the computational complexity of neural-MQ (Sec.~\ref{sec:neural_MQ}) requires $I$ GD steps, in which each $i$-th gradient $\nabla_{r_{1:M}} \sum_{n=1}^N \text{EI}_n(x, f(\sigma_{\tau_i}(r_{1:M})|\theta_{1:M})) $ is computed at once for all $M$ RUs. While under sufficiently large $I$, such GD updates will converge to the (local) minimum of the sum-EI criterion, such gradient computation may not be the best choice under finite GD updates. For instance, imagine we can only update once $(I=1)$ due to computation power constraint at DU. In such case, evaluating gradient of each RU separately, i.e., $\nabla_{r_{m}} \sum_{n=1}^N \text{EI}_n(x, f(\sigma_{\tau_i}(r_{1:M})|\theta_{1:M})) $ for RU $m$, then updating $r_m$, does not necessarily decrease the sum-EI criterion,  since the other RUs $m' \neq m$ are also separately updating their own $r_{m'}$ based on their own gradients $\nabla_{r_{m'}} \sum_{n=1}^N \text{EI}_n(x, f(\sigma_{\tau_i}(r_{1:M})|\theta_{1:M}))$. In this regard, it becomes beneficial to consider \emph{sequential} gradient application where $r_m$ is updated in a sequential way by following a pre-determined ordering. Particular choice of the ordering will be described in the end of this section.

% First, without loss of generality, let us assume that $m=1,2, ..., M$ follows the desired ordering. Then, denoting as $r^{(i)}_{1:M}=(r^{(i)}_1,...,r^{(i)}_M)$ the (relaxed) bits for all RUs at  iteration $i$, we first update the (relaxed) bits for the first RU from $r_1^{(i)}$ to $r_1^{(i+1)}$, i.e., 
%  \begin{align} \label{eq:SGD_for_neural_MQ}
%         r_{1}^{(i+1)} =   r_{1}^{(i)}- \eta \cdot \nabla_{r_1^{(i)}} \sum_{n=1}^N \text{EI}_n(x, f(\sigma_{\tau_i}(r^{(i)}_{1:M})|\theta_{1:M})). 
% \end{align}
%  Then we continue to update by following the order $m=2,3,...,M$, hence the update rule of DU in the $m$-th order follows 
%  \begin{align} \label{eq:SGD_for_neural_MQ}
%         r_{m}^{(i+1)} &=   r_{m}^{(i)}- \eta \cdot \nabla_{r_{m}^{(i)}} \sum_{n=1}^N \text{EI}_n(x, f(\sigma_{\tau_i}(r_{1:M}^{(i,m)})|\theta_{1:M})), 
% \end{align}
% where we have denoted as $r^{(i,m)}_{1:M}=(r^{(i+1)}_1,...,r^{(i+1)}_{m-1},r^{(i)}_{m},...,r^{(i)}_M)$ the updated (relaxed) bits up to ($m-1$)-th RU. It is worth noting that such sequential GD updates require exactly the same number of updates in terms of (relaxed) bits, with the only additional computational complexity raised from $M-1$ additional sum-EI criterion evaluations (\ref{eq:new_EI}), which becomes negligible when adopting large neural networks.  Overall procedure of sequential neural-MQ is summarized in Algorithm~\ref{alg:Seq_neural_MQ}.

% In a manner similar to SMQ in Sec.~\ref{sec:smq} \cite{lee2016multivariate}, the choice of the ordering sequence can affect the final performance in case each RU has different level of influence to the other RUs. To this end, we revisit the interference graph definition (\ref{eq:interference_graph_2})  of $\alpha$-PMQ  to define the sequence as the descending ordering of the \emph{sum interference} $\sum_{m' \neq m} G_m^T G_{m'}$. Accordingly, the first RU in the sequence will have the maximum sum interference, i.e.,  $ \arg\max_{m} \sum_{m' \neq m} G_m^T G_{m'}$; while the last RU in the sequence will have the minimum sum interference, i.e.,  $ \arg\min_{m} \sum_{m' \neq m} G_m^T G_{m'}$. Intuitively, sequential neural-MQ starts updating the (relaxed) bits for the RU that has the most significant influence to the other RUs, hence determining the dominant interference term, so that the following updates for the other RUs can focus on more fine-grained interference controls. 



% % \begin{align}
% %     \label{eq:interference_graph_2}
% %     (m, m') \in \mathcal{E}_\alpha \text{ if } G_m^T G_{m'} > g(\alpha) \text{ and } m \neq m',
% % \end{align}



% \begin{algorithm}[t!] \label{alg:Seq_neural_MQ}
%     \caption{Sequential Neural-MQ}
%     \SetKwInOut{Input}{Input}
%     \Input{Number of iterations $I$; neural codebook $f_m(\cdot)$ for $m=1,...,M$, symbol vector $s$; channel matrix $H=[H_1^\top, ..., H_N^\top]^\top$; precoding matrix $W=[W_1,...,W_N]$; receive beamforming matrix $F=[F_1, ..., F_N]$; step size $\eta > 0$ }
%     \SetKwInOut{Output}{Output}
%     \Output{Discrete bits $b_{1:M}$}
%     \textbf{Initialize} $r_{1:M}$ as the all-zero vectors; Re-index RUs so that $m=1,...,M$ follows the desired ordering;  $\tau_1 = 1$
    
%     \For{\emph{$i=1,...,I$}}{
%     \For{\emph{$m=1,...,M$}}{
%     \begin{align} \label{eq:GD_for_neural_MQ_seq}
%         r_{m} &\leftarrow   r_{m} - \eta \cdot \nabla_{r_{m}} \sum_{n=1}^N \text{EI}_n(x, f(\sigma_{\tau_i}(r_{1:M})|\theta_{1:M})) 
%     \end{align}
%     }update sigmoid temperature $\tau_i = \exp(-5 \cdot i/ I) $}

%     obtain discrete binary messages $b_{1:M}$ in (\ref{eq:neural_hard_b})
    
%     \textbf{Return} $ b_{1:M}$ \\
%     \end{algorithm}


% %Neural-MQ proposed in Sec.~\ref{sec:neural_MQ} computes gradient of each RU $m$ at each iteration $i=1,...,I$ without awareness of the other RUs. In other words, 


% }


==> Sections/4_tree_MQ.tex <==
%\section{Outline of this Report}
%In this report, we make clear analysis on the computational complexity required by the multivariate quantization process.

\section{Tree-MQ}\label{sec:tree_MQ}
In this section, we propose \emph{tree-MQ}, an efficient multivariate quantization scheme that reduces the complexity of MQ by replacing the exhaustive search carried out by MQ over all codewords with a tree-based search \cite[Ch. 12]{gersho2012vector}. In particular, as we will discuss, the complexity of quantization is reduced from order $\mathcal{O}(2^{\sum_{m=1}^M B_m})$ to $\mathcal{O}(2^M \cdot \max_{m=1,...,M}{B_m})$, while we recall that SMQ reduces the complexity from order $\mathcal{O}(2^{\sum_{m=1}^M B_m})$ to $\mathcal{O}(\sum_{m=1}^M 2^{B_m})$. Tree-MQ is agnostic to the topology of the network, not leveraging possible efficiency gains  attainable from the connectivity patterns between UEs and DUs. A topology-aware strategy will be introduced in the next section. 




\begin{figure*}[h]
 \begin{center}\includegraphics[scale=0.28]{Figs/tree_cartoon.pdf}
   \end{center}
   \caption{Background: Illustration of the classical tree-structured quantization. We assume $B=3$ in this figure. (a) Auxiliary codebooks $\hat{\mathcal{X}}^{(1)},...,\hat{\mathcal{X}}^{(B-1)}$ as well as the codebook $\hat{\mathcal{X}}=\hat{\mathcal{X}}^{(B)}$ are given with increasing sizes $|\hat{\mathcal{X}}^{(1)}|=2<|\hat{\mathcal{X}}^{(2)}|=2^2< \cdots <  |\hat{\mathcal{X}}^{(B)}|=2^B=|\hat{\mathcal{X}}|$. (b) Tree-structured quantization starts by comparing input $x$ with first auxiliary codebook $\hat{\mathcal{X}}^{(1)}$. (c) At the second step, based on the previously chosen auxiliary codeword $\hat{x}^{(1)}$, search is refined to the subset $\hat{\mathcal{X}}^{(2)}(\hat{x}^{(1)})$ of two codewords in the second auxiliary codebook $\hat{\mathcal{X}}^{(2)}$. (d) The procedure continues in the same way until step $B$ to yield $\hat{x}=\hat{x}^{(B)}$. }
   \label{fig:tree_prelim}
\end{figure*}
\subsection{Background: Tree-Structured Quantization}
  

We start by reviewing \emph{tree-structured quantization}, one of the most popular schemes for constrained quantization \cite[Ch. 12]{gersho2012vector}.  To this end, we focus here on quantization using a single codebook $\hat{\mathcal{X}}$ with $|\hat{\mathcal{X}}|=2^B$ codewords. Given an input $x$, the quantized signal $\hat{x}$ is obtained by solving the problem  \begin{align} \label{eq:goal_tree}
  \hat{x} = \arg\min_{\hat{x} \in \hat{\mathcal{X}}} ||x-\hat{x}||^2,
\end{align} requiring $|\hat{\mathcal{X}}|$ comparisons of the input signal with each of the codewords. Tree-structured quantization reduces the search complexity by leveraging a specific tree-based structure for the codebook. 

Specifically, tree-structured quantization creates $B-1$ auxiliary codebooks $\{\hat{\mathcal{X}}^{(b)}\}_{b=1}^{B-1}$ with increasing sizes $|\hat{\mathcal{X}}^{(1)}|=2<|\hat{\mathcal{X}}^{(2)}|=2^2< \cdots <  |\hat{\mathcal{X}}^{(B)}|=2^B=|\hat{\mathcal{X}}|$, where the $B$-th codebook coincides with the quantization codebook $\hat{\mathcal{X}}$. Accordingly, each codebook $\hat{\mathcal{X}}^{(b)}$ can be thought of as refining the \emph{resolution} of the previous codebook $\hat{\mathcal{X}}^{(b-1)}$.

Each codeword $\hat{x}^{(b)} \in \hat{\mathcal{X}}^{(b)}$ is associated with a subset of $\hat{\mathcal{X}}^{(b+1)}(\hat{x}^{(b)})$ of two codewords in the next codebook $\hat{\mathcal{X}}^{(b+1)}$. As illustrated in Fig.~\ref{fig:tree_prelim}(a), the subsets $\hat{\mathcal{X}}^{(b+1)}(\hat{x}^{(b)})$ for $\hat{x}^{(b)} \in \hat{\mathcal{X}}^{(b)}$ are disjoint and $\hat{\mathcal{X}}^{(b+1)}=\bigcup_{\hat{x}^{(b)} \in \hat{\mathcal{X}}^{(b)}} \hat{\mathcal{X}}^{(b+1)}(\hat{x}^{(b)})$. 

Search is done sequentially over $B$ steps indexed as $b=1,...,B$, such that at the $b$-th step, tree-structured quantization aims at finding $\hat{x}^{(b)}$, the (auxiliary) quantized output chosen from the $b$-th (auxiliary) codebook $\hat{\mathcal{X}}^{(b)}$. Given the previously chosen auxiliary codeword $\hat{x}^{(b-1)}$ in the $(b-1)$-th auxiliary codebook $\hat{\mathcal{X}}^{(b-1)}$, search at $b$-th step is limited to the \emph{subset} of two codewords in the $b$-th (auxiliary) codebook $\hat{\mathcal{X}}^{(b)}(\hat{x}^{(b-1)})$.



Accordingly, at the $b$-th step, tree-structured quantization solves the problem 
\begin{align} \label{eq:tree_conven_quan}
  \hat{x}^{(b)}=\argmin_{\hat{x}\in \hat{\mathcal{X}}^{(b)}(\hat{x}^{(b-1)})  } ||x-\hat{x}||^2,
\end{align}
which has constant complexity requiring only two comparisons. In \eqref{eq:tree_conven_quan}, we set $\hat{\mathcal{X}}^{(1)}(\cdot) =\hat{\mathcal{X}}^{(1)}$. The final decision is made at the $B$-th step, i.e.,  $\hat{x} = \hat{x}^{(B)}$. Complexity is linear in the number of bits, $B$, instead of the exponential complexity in $B$ for unstructured codebook.


Optimization of the codebooks $\{\hat{\mathcal{X}}^{(d)}\}_{d=1}^D$ is done by applying the Lloyd-Max algorithm in a sequential manner \cite[Ch. 12]{gersho2012vector}, so that the $b$-th codebook is obtained by solving 
\begin{align}
  \min_{\hat{\mathcal{X}}^{(b)}} \mathbb{E}_x \big[||x - \hat{x}^{(b)}||^2\big],
\end{align}
given the previously optimized codebooks $\{\hat{\mathcal{X}}^{(b')}\}_{b'=1}^{B-1}$, where the quantized output $\hat{x}^{(b)}$ is evaluated using \eqref{eq:tree_conven_quan}. In practice, expectation is approximated by empirical averaging over available training examples. The performance degradation of tree-structured quantization as compared to unstructured quantization depends highly on the statistics of the input signal $x$, and is generally hard to quantify \cite[Ch. 12]{gersho2012vector}. 




\begin{algorithm}[t!] \label{alg:tree}
  \caption{Tree-Structured Quantization}
  \SetKwInOut{Input}{Input}
  \Input{Codebook $\hat{\mathcal{X}}$; depth $B$; $B-1$ auxiliary codebooks $\hat{\mathcal{X}}^{(1)},...,\hat{\mathcal{X}}^{(B-1)}$; channel matrix $H$, precoding matrix $W$, input symbol vector $s$ }
  \SetKwInOut{Output}{Output}
  \Output{Quantized output $\hat{x}$}
  \textbf{Set} $\hat{\mathcal{X}}^{(B)}=\hat{\mathcal{X}}$, $\hat{\mathcal{X}}^{(1)}(\cdot)=\hat{\mathcal{X}}^{(1)}$ \\
  \For{\emph{$b=1,...,B$}}{
    Solve the problem \eqref{eq:tree_conven_quan}, i.e., 
    \begin{align} 
      \hat{x}^{(b)}=\argmin_{\hat{x}\in \hat{\mathcal{X}}^{(b)}(\hat{x}^{(b-1)})  } ||x-\hat{x}||^2. \nonumber
    \end{align}
  }
  \textbf{Return} $\hat{x}^{(B)}$ \\
  \end{algorithm}

  




\subsection{Tree-MQ}
Recall that computational complexity of MQ is $\mathcal{O}(2^{\sum_{m=1}^M B_m})$ due to the exhaustive search over the $M$ codebooks $\hat{\mathcal{X}}_{1:M} = \{ \hat{\mathcal{X}}_m \}_{m=1}^M $, each with size $2^{B_m}$, when solving problem \eqref{eq:obj_MQ_sota}. Tree-structured quantization in the previous subsection can be applied for each $m$-th DU, such that \emph{resolution refinement} takes place for each DU separately. In the following, we will assume that the fronthaul capacity for every DU is same, i.e., $B_m=B$ for $m=1,...,M$, so that every DU has the same number of codewords. This allows for every DU to adopt the same tree structure. Generalization to the case of different fronthaul capacties will be discussed in the latter part of this subsection.

Given $B-1$ auxiliary codebooks $\hat{\mathcal{X}}_m^{(1)},...,\hat{\mathcal{X}}_m^{(B-1)}$ for each DU $m$, tree-MQ solves at each $b$-th step the problem
\begin{align} \label{eq:tree_mq}
  \hat{x}^{(b)}=\argmin_{\hat{x}\in \hat{\mathcal{X}}_{1:M}^{(b)} (\hat{x}^{(b-1)}) } \sum_{n=1}^N \text{EI}_n (\hat{x}),
\end{align}
where we have defined the restricted codebook $\hat{\mathcal{X}}^{(b)}(\hat{x}^{(b-1)})$ as in the previous subsection and $\hat{\mathcal{X}}_{1:M}^{(b)}(\hat{x}^{(b-1)})$ represents the Cartesian product of the restricted codebooks across all DUs. 

Tree-MQ has a complexity of order $\mathcal{O}(2^M)$ at each $b$-th step, since the joint optimization \eqref{eq:tree_mq} is over a space of dimension $2^M$, corresponding to $M$ combination of the two codewords in all restricted codewords $\hat{\mathcal{X}}_{1:M}^{(b)}(\hat{x}^{(b-1)})$. Therefore, the overall complexity is $\mathcal{O}(2^M\cdot B)$. Tree-MQ is illustrated in Fig.~\ref{fig:tree_mq}. 


Optimization of the codebooks $\{\{\hat{\mathcal{X}}_m^{(d)}\}_{d=1}^B\}_{m=1}^M$ is done again by applying Lloyd-Max algorithm in a sequential manner akin to the tree-structured quantization described in the previous section. Accordingly, given fixed precoding $W$, the $d$-th codebook is obtained by addressing the problem 
\begin{align}
  \label{eq:obj_tree_mq_codebook}
  \min_{\hat{\mathcal{X}}^{(d)}_{1:M}} \mathbbm{E}_{H,s}\bigg[ \sum_{n=1}^N \Big| H_n (\hat{x}^{(b)}-W_{n}s_n ) \Big|^2 \bigg],
\end{align}
with $\hat{x}^{(b)}$ the solution of the tree-MQ problem (\ref{eq:tree_mq}), and  the expectation term $\mathbbm{E}_{H,s}[\cdot]$ in \eqref{eq:obj_wonju_codebook} is approximated by an empirical average using realizations of channels and symbol vectors from the respective distributions. 

Until now, we have assumed that every DU has the same fronthaul capacity. When the DUs have different fronthaul capacities, one can simply set the restricted codebooks $\hat{\mathcal{X}}_m^{(b)}(\hat{x}_m^{(b-1)})$ as $\hat{\mathcal{X}}_m^{(b)}(\hat{x}_m^{(b-1)})=\hat{\mathcal{X}}_m^{(b-1)}(\hat{x}_m^{(b-2)})$ for all $b > B_m$ and $m=1,...,M$. The complexity order is $\mathcal{O}(2^M \cdot \max_{m=1,...,M}B_m)$.


\begin{figure}[h]
  \begin{center}\includegraphics[scale=0.51]{Figs/tree_mq.pdf} 
    \end{center}
    \caption{Tree-MQ has complexity of $\mathcal{O}(B\cdot 2^M)$. The circles represent the (auxiliary) codewords within the (auxiliary) codebooks of the DUs. In tree-MQ, the CU selects the auxiliary codeword $\hat{x}^{(1)}$ for all $M$ DUs at the first step. Then, the CU chooses the auxiliary codeword $\hat{x}^{(2)}$ at the second step based on the previously chosen auxiliary codeword $\hat{x}^{(1)}$. And the procedure continues in the same way until step $B$ to yield $\hat{x}=\hat{x}^{(B)}$.}
    \label{fig:tree_mq}
 \end{figure}


\begin{algorithm}[t!] \label{alg:tree_mq}
  \caption{Tree-Structured Multivariate Quantization}
  \SetKwInOut{Input}{Input}
  \Input{Codebook $\hat{\mathcal{X}}_{1:M}$; $B-1$ auxiliary codebooks for all DUs  $\{\{\hat{\mathcal{X}}_m^{(d)}\}_{d=1}^B\}_{m=1}^M$; channel matrix $H$, precoding matrix $W$, input symbol vector $s$  }
  \SetKwInOut{Output}{Output}
  \Output{Quantized output $\hat{x}$}
  \textbf{Set} $\hat{\mathcal{X}}_m^{(B)}=\hat{\mathcal{X}}_m$, $\hat{\mathcal{X}}_m^{(1)}(\cdot) = \hat{\mathcal{X}}_m^{(1)}$ for $m=1,...,M$ \\
  \For{\emph{$b=1,...,B$}}{
    Solve the problem \eqref{eq:tree_mq}, i.e., 
    \begin{align} \nonumber
      \hat{x}^{(b)}=\argmin_{\hat{x}\in \hat{\mathcal{X}}_{1:M}^{(b)} (\hat{x}^{(b-1)}) } \sum_{n=1}^N \text{EI}_n (\hat{x}).
    \end{align}
  }
  \textbf{Return} $\hat{x}^{(B)}$ \\
  \end{algorithm}






==> Sections/5_b_overhead_comp.tex <==
\section{Fronthaul Overhead Analysis}\label{sec:overhead_comp}

In this section, we present an analysis of the fronthaul overhead of PC as compared to conventional CP schemes. This will support the performance comparison between PC and CP in the next section. 

Assume transmission using an OFDM radio interface with  $N_\text{RB}$ resource blocks (RBs), in which each RB consists of  $N_\text{OFDM}$ OFDM symbols and $N_\text{SC}$ subcarriers. The total number of resource elements (REs), or channel uses, is denoted as 
\begin{align}
    N_\text{RE}=N_\text{RB}\cdot N_\text{OFDM}\cdot N_\text{SC}.
\end{align}
Recall that in the previous sections, we have focused on any one such channel use. 



CP schemes apply the same precoding matrix across $N_\text{REP}$ resource elements, typically a multiple of $N_\text{OFDM}\cdot N_\text{SC}$, to reduce the fronthaul overhead. Furthermore, they transmit all the information bits to all DUs. Defining as $B_\text{CP}$ the number of bits used to compress each element of the precoding matrix $W$, the fronthaul overhead for each  channel use, i.e., for each RE, is given by 
\begin{align}
    \label{eq:B_CP}
    B_m =  \underbrace{R_\text{sum}}_{\substack{\text{sum-rate}\\\text{(bit/channel use)}}} +  \underbrace{N_m^\text{tx}\cdot L\cdot B_\text{CP}}_{\text{precoding quantization}} \cdot \frac{1}{N_\text{REP}},
\end{align}
where the division by $N_\text{REP}$ reflects the fronthaul capacity saving due to the reuse of the precoding matrix across $N_\text{REP}$ channel uses. Note the dependence on the sum-rate $R_\text{sum}$ given the need to communicate all information bits to the DUs. 

In contrast, the fronthaul overhead of the PC scheme is given by the selected number $B_m$ of bits per channel use as discussed in Sec.~\ref{sec:sys_model}. Accordingly, the dependence of the fronthaul overhead on the sum-rate, on the number of data streams $L$, and on the number of antennas $N_m^\text{tx}$  is indirect, and PC generally can operate in lower fronthaul capacity regimes as compared to CP. 


==> Sections/6_Experimental_Results.tex <==
\section{Experimental Results} \label{sec:experiments}
In this section, we compare the proposed PC schemes with CP scheme. We first compare the proposed PC schemes, tree-MQ and $\alpha$-PMQ, with respect to conventional PC schemes, namely SMQ, MQ, \cite{lee2016multivariate}, and PtPQ. Then we provide a comparison between PC ans CP. 


Hyperparameters for PC schemes in \eqref{eq:regularized_EI}  are set as $(\beta,\gamma)=(1,0)$ for $B_m \leq 10$ and as $(\beta,\gamma)=(0,1)$ for $B_m > 10$. We set the average signal-to-noise ratio (SNR) for each DU as $P/\sigma^2=10 \text{ dB}$ unless specified otherwise.






% Regarding OFDM radio interface, we set the subcarrier spacing as $30$ kHz with $N_\text{RB}=273$ RBs each with $N_\text{OFDM}=14$ OFDM symbols and $N_\text{SC}=12$ subcarriers. We design the precoding matrix $W$ based on the weighted minimum mean square error (WMMSE) algorithm \cite{feng2021weighted}, unless specified otherwise. 



%We adopt zero-forcing precoding. %and that there are $N=10$ single-antenna UEs. {\color{blue} We will consider multi-antenna UEs in the next subsection}. We assume 3GPP urban macrocell (UMa) setting to model the channel matrix $H$. We adopt zero-forcing precoding.


% \begin{figure}[h]
%   \begin{center}\includegraphics[scale=0.46]{Figs/sys_uma.pdf}
%     \end{center}
%     \caption{Assumed communication environment in a single cell: Each DU is equipped with $N_m^\text{tx}=4$ antennas to serve $N=10$ single-antenna UEs. (a) $M=4$ DUs with fronthaul capacity $B_m=3$ bits per symbol; (b) $M=6$ DUs with fronthaul capacity $B_m=2$ bits per symbol. 3GPP urban macrocell (UMa) \cite{3gpp} is assumed for channel modelling.}
%     \label{fig:sys_experiment_uma}
%  \end{figure}
 
 
 \begin{figure}[h]
  \begin{center}\includegraphics[scale=0.18]{Figs/M_6_single.png}
    \end{center}
    \caption{Spectral efficiency as a function of (top) normalized total computational complexity (bottom) normallized parallel computational complexity. We assume  $M=6$ DUs equipped with $N_m^\text{tx}=4$ antennas under fronthaul capacity $B_m=2$ and $N=10$ single-antenna UEs. Reported values are averaged over $100$ different channel realizations with $100$ different symbols per channel realization. For both training and testing, the same, fixed, large scale parameters \cite{3gpp} of DUs and UEs are assumed. }
    \label{fig:results_tree_and_pmq}
 \end{figure}

  
 \begin{figure}[h]
  \begin{center}\includegraphics[scale=0.18]{Figs/M_4_single.png}
    \end{center}
    \caption{Spectral efficiency as a function of (top) normalized total computational complexity (bottom) normallized parallel computational complexity. We assume  $M=4$ DUs equipped with $N_m^\text{tx}=4$ antennas under fronthaul capacity $B_m=3$ and $N=10$ single-antenna UEs. Reported values are averaged over $100$ different channel realizations with $100$ different symbols per channel realization. For both training and testing, the same, fixed, large scale parameters \cite{3gpp} of DUs and UEs are assumed. }
    \label{fig:results_tree_and_pmq_2}
 \end{figure}
 


\subsection{Computational Complexity Analysis}
First, we study the impact of the computational complexity of fronthaul quantization on the spectral efficiency. We consider two metrics: (\emph{i}) the \emph{total number of operation}, with one operation unit corresponding to the evaluation of the EI in \eqref{eq:EI_multi_antenna}; and (\emph{ii}) the \emph{number of operations on a parallel processor}, whereby parallel operation at different subprocessors are counted only once. Table~\ref{table:tab_comp_comp} reviews the complexity measures for all schemes assuming $B_m=B$ for all DUs $m=1,...,M$. In the table, we evaluate the total computational complexity of $\alpha$-PMQ by defining the number of iterations as $T$ and the average number of DUs included in an iteration as $M'$.  


In order to optimize the codebook, for all schemes, we assume the availability of $100$ different channel realizations with $100$ different symbols per channel realization, and the symbols for each UE are generated by complex standard normal distribution $\mathcal{CN}(0,1)$ as in \cite{lee2016multivariate}. We adopt zero-forcing precoding,  while assuming that each DU has $N_m^\text{tx}=4$ antennas. The channel follows the  3GPP urban macrocell channel model. 


\begin{table}
  \caption{Computational complexity in terms of total number of operation and number of operations on a parallel processor ($T$ is the number of iterations of $\alpha$-PMQ and $M' \leq M$ is the average number of DUs included in each step)}
  \label{table:tab_comp_comp}
  \centering
  \begin{tabular}{l|l|l}
    scheme & total & parallel \\ 
    \midrule
    PtPQ & $M \cdot 2^B$  & $2^B$     \\
    MQ     & $2^{MB}$ & $2^{MB}$      \\
    SMQ     & $M\cdot 2^B$      & $M\cdot 2^B$ \\
    tree-MQ     & $B\cdot 2^M$      &  $B\cdot 2^M$ \\
    $\alpha$-PMQ     & $T \cdot M'\cdot 2^B$      & $T\cdot 2^B$  \\
  \end{tabular}
\end{table}


\subsubsection{Single-Antenna UE}
First, we assume $N=10$ single antenna UEs with $L_n=1$ transmit symbol per each UE. In Fig.~\ref{fig:results_tree_and_pmq}, we consider $M=6$ DUs with fronthaul capacity $B_m=2$, and in Fig.~\ref{fig:results_tree_and_pmq_2} we consider $M=4$ DUs with fronthaul capacity $B_m=3$. We set $\alpha=0.5$ for $\alpha$-PMQ, and we vary the complexity of $\alpha$-PMQ by increasing the number $T$ of iteration. Accordingly, all schemes but $\alpha$-PMQ provide a single point in the performance-complexity trade-off.  The complexity is shown after normalization by the reference complexity of PtPQ, and the spectral efficiency is computed using \eqref{eq:sum_rate_single}.

Tree-MQ outperforms SMQ \cite{lee2016multivariate} at the cost of a larger computational complexity. $\alpha$-PMQ outperforms both tree-MQ and SMQ in terms of spectral efficiency. Furthermore, in the presence of a parallel processor, the performance improvement is obtained at a lower computational complexity. Specifically, with a parallel processor, for a fixed spectral efficiency, $\alpha$-PMQ has lowest computational complexity; while for a fixed computational complexity, $\alpha$-PMQ has the highest spectral efficiency.


The spectral efficiency benefits of $\alpha$-PMQ hinge on the possibility to isolate the groups of DUs with limited mutual interference. Accordingly, for more complex systems, such as that considered in Fig.~\ref{fig:results_tree_and_pmq} as compared to Fig.~\ref{fig:results_tree_and_pmq_2}, $\alpha$-PMQ exhibits the largest performance gains. Furthermore, as discussed, the computational complexity savings of $\alpha$-PMQ are realized when  allowing for parallel computations across multiple DUs, i.e., $M'=1.88$ for Fig.~\ref{fig:results_tree_and_pmq}, and $M'=1.68$ for Fig.~\ref{fig:results_tree_and_pmq_2}.



\begin{figure}[h]
  \begin{center}\includegraphics[scale=0.18]{Figs/multi_ant_UE_M_6.png}
    \end{center}
    \caption{Spectral efficiency as a function of (left) normalized total computational complexity (right) normallized parallel computational complexity. We assume  $M=6$ DUs equipped with $N_m^\text{tx}=4$ antennas under fronthaul capacity $B_m=2$ and $N=5$ multi-antenna UEs ($N_n^\text{rx}=2)$. Reported values are averaged over $100$ different channel realizations with $100$ different symbols per channel realization. For both training and testing, the same, fixed, large scale parameters \cite{3gpp} of DUs and UEs are assumed. }
    \label{fig:multi_M_6}
 \end{figure}

  
 \begin{figure}[h]
  \begin{center}\includegraphics[scale=0.18]{Figs/multi_ant_UE_M_4.png}
    \end{center}
    \caption{Spectral efficiency as a function of (left) normalized total computational complexity (right) normallized parallel computational complexity. We assume  $M=4$ DUs equipped with $N_m^\text{tx}=4$ antennas under fronthaul capacity $B_m=3$ and $N=5$ multi-antenna UEs ($N_n^\text{rx}=2)$. Reported values are averaged over $100$ different channel realizations with $100$ different symbols per channel realization. For both training and testing, the same, fixed, large scale parameters \cite{3gpp} of DUs and UEs are assumed. }
    \label{fig:multi_M_4}
 \end{figure}
 

The conclusion reached via Fig.~\ref{fig:results_tree_and_pmq} and Fig.~\ref{fig:results_tree_and_pmq_2} are confirmed in Fig.~\ref{fig:multi_M_6} and Fig.~\ref{fig:multi_M_4}, where we consider a system with $N=5$ multi-antenna UEs equipped with $N_n^\text{rx}=2$, with $L_n=2$ complex symbols intended for each user. The other settings for Fig.~\ref{fig:multi_M_6} and Fig.~\ref{fig:multi_M_4} are same as in Fig.~\ref{fig:results_tree_and_pmq} and Fig.~\ref{fig:results_tree_and_pmq_2}, respectively.






\subsection{Comparison between CP and PC for a Small-Scale System}
In this subsection, we focus on the comparison between CP and PC schemes, including also the case with  infinite fronthaul capacity as a benchmark. We consider again the 3GPP urban micro cell channel model, assuming a subcarrier spacing of $30$ kHz. The precoding matrix for all schemes is designed based on the WMMSE algorithm \cite{feng2021weighted}. In particular, for CP, precoding is shared across $N_\text{REP}=48$ subcarriers (with $N_\text{OFDM}=1$), and the WMMSE algorithm is applied by using the channel matrix of the central RE for the given set of $N_\text{REP}$ REs. Furthermore, for CP we adopt scalar uniform quantization codebooks, while for PC quantization codewords were generated at random via uniform sampling over the $(N_m^\text{tx}-1)$-sphere with radius $\sqrt{P}$. This allows us to focus solely on the advantages due to quantization, not relying on codebooks tailored to specific channel conditions. 

We have  $M=4$ DUs with $N_m^\text{tx}=8$ antennas and $N=10$ UEs with $N_n^\text{rx}=2$ antennas. We further assume $L_n=1$ data stream for each UE $n$, and set SNR per DU as $1$ dB. 

We study  in Fig.~\ref{fig:cp_pc_ser} and Fig.~\ref{fig:cp_pc_sum_rate} the symbol error rate (SER) and sum-spectral efficiency as a function of per-channel use fronthaul capacity $B$, assumed to be the same for all DUs. The SER is plotted by assuming uncoded $8$-PSK transmission so that the sum-rate in \eqref{eq:B_CP} is given by $R_\text{sum}=3 N$. For the sum-spectral efficiency, we estimated the effective interference-plus-noise covariance matrix $K_e = \mathbb{E}[(\hat{s}_n-s_n)(\hat{s}_n-s_n)^\dagger]$, where the estimated symbol vector $\hat{s}_n$ at UE $n$ is obtained by applying the MMSE receiver to the received signal $y_n$ \eqref{eq:rx_multi}. This allows us to use the standard capacity formula $\log \det (K_s + K_e) - \log \det (K_e)$, with signal covariance $K_s = \mathbb{E}[s_n s_n^\dagger]$. We have estimated the covariance  terms via averaging over $1000$ independent transmissions.

For the case of uncoded transmission studied in Fig.~\ref{fig:cp_pc_ser}, the CP scheme requires at least $3N+N_m^\text{tx}\cdot L \cdot B_\text{CP}/N_\text{REP} > 30$ bits per-channel use on the fronthaul by \eqref{eq:B_CP}, while PC scheme can operate with lower fronthaul capacities. Furthermore,  PC schemes attain the same SER performance of a scheme with  infinite fronthaul capacity, while the CP scheme suffers from a higher SER due to the shared codebook across $N_\text{RBE}=48$ subcarriers. The performance levels of all PC schemes coincide for sufficiently large $B$, due to the use of objective \eqref{eq:regularized_EI} with $\beta=0$ and $\gamma=1$. 
%Both CP and PC schemes attain the SER performance of an infinite fronthaul capacity scheme given a sufficiently high fronthaul capacity. 

In Fig.~\ref{fig:cp_pc_sum_rate}, we compare the sum-spectral efficiency for CP and PC schemes. In a manner similar to Fig.~\ref{fig:cp_pc_ser}, CP is inapplicable for low values of the fronthaul capacity, while PC can operate at lower fronthaul capacities, outperforming CP in all fronthaul capacity regimes.


 \begin{figure}[h]
\begin{center}\includegraphics[scale=0.12]{Figs/cp_pc_comp_ser.png}
    \end{center}
    \caption{Per-channel symbol error rate  as a function of per-channel use fronthaul capacity $B$. The lowest symbol error rate among the  $N=10$ UEs is shown. $M=4$ DUs with $N_m^\text{tx}=8$ antennas and $N=10$ UEs with $N_n^\text{rx}=2$ antennas are assumed.  Each UE decodes $L_n=1$ 8-PSK complex symbol. All PC schemes share the same random codebook uniformly sampled in $7$-sphere with radius $\sqrt{P}=1$ (noise variance set $\sigma^2=1$). }
    \label{fig:cp_pc_ser}
 \end{figure}



 \begin{figure}[h]
\begin{center}\includegraphics[scale=0.12]{Figs/cp_pc_sum_rate.png}
    \end{center}
    \caption{Per-channel  sum spectral efficiency  as a function of per-channel use fronthaul capacity $B$. $M=4$ DUs with $N_m^\text{tx}=8$ antennas and $N=10$ UEs with $N_n^\text{rx}=2$ antennas are assumed.  All PC schemes share the same random codebook uniformly sampled in $7$-sphere with radius $\sqrt{P}=1$ (noise variance set $\sigma^2=1$). }
    \label{fig:cp_pc_sum_rate}
 \end{figure}




\subsection{Comparison between CP and PC for a Large-Scale System}
Finally, we compare the performance of CP and PC for a larger-scale system with  $M=12$ DUs, each with  $N_m^\text{tx}=8$ antennas, and $N=8$ UEs with $N_n^\text{rx}=4$ antennas. The number of data streams per UE is $L_n=2$. For CP, we assume a standard setting in which the same precoding matrix is reused across $N_\text{REP}=12 \cdot 14 \cdot 4$ channel uses, with 12 being the number of subcarriers and 4 the number of OFDM symbols, and 
$B_\text{CP}=16$ bits are used per precoding element. By (\ref{eq:B_CP}), this requires fronthaul capacity of $B=67$ for $16$-QAM transmission.   Pedestrian UEs with velocity $3 $ km/h \cite{3gpp_ped} are assumed. The other settings are same as in Fig.~\ref{fig:cp_pc_ser} and Fig.~\ref{fig:cp_pc_sum_rate}.  

In order to simplify the quantization step \eqref{eq:obj_MQ_sota}, for fronthaul capacity values $B$ larger than 16, we adopt a simple  uniformly spaced per-channel use quantization codebook. This allows us to address problem \eqref{eq:obj_MQ_sota} via a sequential approach based on lattice decoding. We note that we expect that significant gains may be obtained with lattice codes that are lifted to cover the sphere of points with power $P$. Engineering such a system is work in progress, with preliminary results shown in the last part of this report. 

% Specifically, the quantization step size $\Delta_m$ for DU $m$ is determined by the predetermined confidence level $\tau \in (0,1)$ as
% \begin{align}
%     \Delta_m = \frac{2\cdot Q^{-1}( (1 -\tau)/2 ) \cdot \sqrt{P/(2\cdot N_m^\text{tx})}}{2^{B_m/2\cdot N_m^\text{tx}}-1},
% \end{align}
% where $Q(\cdot)$ is the Q-function, i.e., $Q(z) = \Pr(Z > z)$ for $Z \sim \mathcal{N}(0,1)$. We set $\tau=0.8, 0.9, 0.95$ for $B_m=64, 128, 256$, respectively. 


Fig.~\ref{fig:cppcmany1} shows sum-spectral efficiency for CP and PC as a function of fronthaul capacity $B$. Aligned with previous results, PC reaches the performance of infinite fronthaul capacity,  while CP scheme can only achieve $60\%$ due to shared precoding across $N_\text{REP}=672$ REs. .

 Lastly, in Fig.~\ref{fig:cppcmany2}, we investigate SER for $16$-QAM transmission. While CP  suffers from SER around $0.5$, PC achieves lower SER of nearly $0.3$ while requiring only $1/3$ of fronthaul capacity that scheme CP requires. With sufficient fronthaul capacity, PC achieves SER of infinite fronthaul case (less than $0.1$). 



 \begin{figure}[h]
\begin{center}\includegraphics[scale=0.28]{Figs/cp_pc_many_1.pdf}
    \end{center}
    \caption{Per-channel  sum spectral efficiency  as a function of per-channel use fronthaul capacity $B$. $M=12$ DUs with $N_m^\text{tx}=8$ antennas and $N=8$ UEs with $N_n^\text{rx}=4$ antennas each carrying $L_n=2$ data streams are assumed. PC scheme adopts random codebook for $B_m \leq 16$ as in Fig.~11 and Fig.~12, while for $B_m > 16$ uniformly spaced quantization codebook is assumed.  }
    \label{fig:cppcmany1}
 \end{figure}


 \begin{figure}[h]
\begin{center}\includegraphics[scale=0.28]{Figs/cp_pc_many_2.pdf}
    \end{center}
    \caption{Per-channel  average SER  as a function of per-channel use fronthaul capacity $B$. $M=12$ DUs with $N_m^\text{tx}=8$ antennas and $N=8$ UEs with $N_n^\text{rx}=4$ antennas each carrying $L_n=2$ data streams are assumed. PC scheme adopts random codebook for $B_m \leq 16$ as in Fig.~11 and Fig.~12, while for $B_m > 16$ uniformly spaced quantization codebook is assumed.  }
    \label{fig:cppcmany2}
 \end{figure}


As mentioned earlier, manipulating lattice codes beyond the simple uniform design has its potential to significantly improve the performance of PC scheme. While still work in progress, we present preliminary results that are obtained by adopting polar coordinate quantizer which effectively lifts the lattice codes so as to cover the sphere. As shown in Fig.~\ref{fig:cppcmany1_polar} and Fig.~\ref{fig:cppcmany2_polar}, the proposed PC with polar coordinate quantizer significantly outperforms PC with uniform quantizer, which again  outperforms CP scheme with an increased margin. 


 \begin{figure}[h]
\begin{center}\includegraphics[scale=0.28]{Figs/cp_pc_many_1_polar.pdf}
    \end{center}
    \caption{Per-channel  sum spectral efficiency  as a function of per-channel use fronthaul capacity $B$. $M=12$ DUs with $N_m^\text{tx}=8$ antennas and $N=8$ UEs with $N_n^\text{rx}=4$ antennas each carrying $L_n=2$ data streams are assumed. PC scheme adopts random codebook for $B_m \leq 16$ as in Fig.~11 and Fig.~12, while for $B_m > 16$ polar coordinate quantization codebook is assumed.  }
    \label{fig:cppcmany1_polar}
 \end{figure}


 \begin{figure}[h]
\begin{center}\includegraphics[scale=0.3]{Figs/cp_pc_many_2_polar.pdf}
    \end{center}
    \caption{Per-channel  average SER  as a function of per-channel use fronthaul capacity $B$. $M=12$ DUs with $N_m^\text{tx}=8$ antennas and $N=8$ UEs with $N_n^\text{rx}=4$ antennas each carrying $L_n=2$ data streams are assumed. PC scheme adopts random codebook for $B_m \leq 16$ as in Fig.~11 and Fig.~12, while for $B_m > 16$ polar coordinate quantization codebook is assumed.  }
    \label{fig:cppcmany2_polar}
 \end{figure}
 



==> Sections/7_Future_Work.tex <==
\begin{itemize}
    \item Graph models are inherently modular:
    \begin{itemize}
        \item can add/remove nodes
    \end{itemize}
    \item Knowledge can be shared across RBs via node filters (e.g., initialization) and/or graph connectivity.
    \item Robustness to imperfect CSI can be ensured via ``uncertainty injection'' at design time \footfullcite{cui2023uncertainty}
\end{itemize}

==> Sections/A_App.tex <==
\section{Proposed Approach}
\subsection{Goal}
In this project, we aim at designing a multivariate quantization scheme that improves the state-of-the-art approach in \cite{lee2016multivariate} by allowing: (\emph{i}) reduced run-time computational complexity, from exponential to linear in the fronthaul sum-rate; (\emph{ii}) consideration of multiple antennas at the DUs; and (\emph{iii}) the optimization of general utility functions dependent on the achievable rates. 

Accordingly, we wish to design a  multivariate quantizer $f^\text{enc}(\cdot|H): \mathcal{C}^{N^\text{tx}_{1:M}\times 1} \rightarrow \{1,...,2^{B_1}\}\times \cdots \times \{1,...,2^{B_M}\}$ that takes input $x$ to output the bits for all DUs; dequantizers for the DUs $m\in[1,...,M]$, $f_m^\text{dec}(\cdot): \{1,...,2^{B_m}\}\ \rightarrow \mathcal{C}^{N^\text{tx}_{m}\times 1}$, each of which  takes the bits for DU $m$ from the fronthaul to output codeword $\hat{x}_m$; and precoding matrix $W(\cdot): \mathcal{C}^{N_{1:M}^\text{tx}\times N}\rightarrow \mathcal{C}^{N_{1:M}^\text{tx}\times N}$ that takes input the channel matrix $H$ and outputs the precoding matrix $W_H$. We wish to address the problem 
% e.g.,  $f^\text{enc}(x|H)=\{j_1,...,j_M\}$, $f^\text{dec}(\{j_1,...,j_M\})=\hat{x}$, {\color{red}$W(H) = (H^\dagger H)^{-1}H$}
\begin{align}
    \label{eq:obj_proposed}
    &\min_{f^\text{enc}(\cdot|H), \{f_m^\text{dec}(\cdot)\}_{m=1}^M, W(\cdot)} \mathbb{E}_{H}\bigg[ \sum_{n=1}^N \alpha_n u_n( \text{SINR}_n(H) ) \bigg],
\end{align}
with instantaneous SINR for UE $n$ defined as
\begin{align}
&\text{SINR}_n(H) = \frac{P \mathbb{E}_{s}\big[|H_n^\dagger W_{n}(H)s_n|^2\big]}{\sigma^2 +P\mathbb{E}_{s}\big[ |H_n^\dagger (\hat{x}-x + \sum\limits_{n' \neq n}W_{n'}(H)s_{n'})|^2\big] }\nonumber \\&\text{ s.t. } \hat{x} = [f_1^\text{dec}(f^\text{enc}(x|H)),..., f_M^\text{dec}(f^\text{enc}(x|H))]^T \text{ with } x = W(H)s,
\end{align}
where $u_n(\cdot)$ is any (non-linear, non-convex) utility function of the achievable rates, e.g., the weighted sum-rate.
%\item Run-time complexity linear in $\sum_{m=1}^M B_m$;
%\item Multi-antenna DU;
%\item Reuse of information across resource blocks (RBs);
%\item Imperfect CSI.

%While using sufficiently rich enough black-box neural network would solve \eqref{eq:obj_proposed} from universal approximation theorem \cite{hornik1991approximation}, in general, a huge amount of training overhead \cite{simeone2022machine} is needed which is inappropriate for wireless communication systems \cite{simeone2020learning}. Moreover, even though such functions have been optimized, general black-box neural networks are not scalable, i.e., cannot be applied for different number of users and/or different number of DUs. To this end, we propose a \textbf{scalable} joint design of precoding and multivariate quantization with \textbf{low-complexity}.

% \subsection{Design Goal}
% The sum-EI criterion can be viewed as an approximation of the sum-rate 
% \begin{align}
%     \mathbb{E}_H \bigg[ \sum_{n=1}^N \alpha_n \log(1+ \text{SINR}_n(H)) \bigg]
% \end{align}
% for $\text{SINR}_n(H) \ll 1$. We consider a general utility function $\sum_{n=1}^N \alpha_n u_n(\text{SINR}_n(H))$ which includes the sum-rate as a special case.

\subsection{Architecture: Fixed Precoding (Phase 2)}
As discussed in the previous section, in reference \cite{lee2016multivariate}, computational complexity was addressed by proposing a sequential compression scheme. However, this approach has theoretical justification only for infinite quantization blocks. For finite blocks, the sequential approach has non-negligible performance loss (see, e.g., Fig. 5 in \cite{lee2016multivariate}), but it is able to reduce computational complexity, which becomes exponential in the maximum fronthaul rate, $\max_n B_n $, rather than in the fronthaul sum-rate.

Inspired by the sequential approach, we propose to adopt a \textbf{modular graph-based multivariate quantizer} at the CU followed by \textbf{separate dequantizers} at the DUs.
\begin{figure}\begin{center}\includegraphics[scale=0.35]{Figs/proposed_architecture.pdf}
   \end{center}
   \caption{Proposed graph-based multivariate quantizer, which depends on the channel realization $H$, and the dequantizers, which does not depend on the channel. }\label{fig:proposed_architecture_graph}
\end{figure}
The graph-based quantizer can be a graph filter or more generally a graph neural network (GNN). As shown in Fig.~\ref{fig:proposed_architecture_graph}, the graph-based quantizer utilizes information from the channel matrix $H$, e.g., as edge information, to enable adaptation to the channel realization. In contrast, the dequantizers do not depend on the channel matrix, and may be linear (codebook) or non-linear (neural networks). The dequantizers are not updated based on channel state information. As anticipated in the previous section, the proposed architecture of the graph-based quantizer can be viewed as a special, novel, type of graph autoencoder \cite{kipf2016variational, tang2022graph}. 

%Recent related work: From graph embedding, mostly aims at reconstructing the graph structure, e.g., adjacency matrix \footfullcite{kipf2016variational} with recent work that focuses on reconstructing node features \footfullcite{tang2022graph}. 




%Using some channel characteristics to GNN ... e.g., edge ... maybe ... angle ... spacity ... 





\subsection{Architecture: Joint Precoding and Multivariate Quantization (Phase 3)}
In the previous subsection (Phase 2), we discussed a scalable, low-complexity multivariate quantization approach given a fixed precoding matrix. In Phase 3, we aim at designing both precoding matrix and graph-based quantizer jointly by addressing problem \eqref{eq:obj_proposed}. To this end, we propose to consider a \textbf{hypernetwork}-based approach, whereby the hypernetwork at the CU takes input as the channel matrix $H$ to output the precoding matrix $W(H)$  \cite{ha2016hypernetworks} without requiring run-time optimization. Specifically, to allow for the joint adaptation of precoding and  multivariate quantization to channel conditions, we will apply hypernetwork also to the graph-based quantizer.  The overall architecture of the proposed joint design of precoding and multivariate quantization is illustrated Fig.~\ref{fig:proposed_overall}.
\begin{figure*}
 \begin{center}\includegraphics[scale=0.25]{Figs/proposed_overall.pdf}
   \end{center}
   \caption{Overall illustration of the proposed scalable, low-complexity multivariate quantization framework.}  
   \label{fig:proposed_overall}
\end{figure*}

% By jointly updating hypernetworks for precoding and quantizer, and the shared dequantizer (which does not depend on the channel), we expect that the proposed solution to significantly reduce the computational complexity at run time with negligible performance loss as compared to the state-of-the-art solution \cite{lee2016multivariate} introduced in Sec.~\ref{sec:sota}. Note again that \cite{lee2016multivariate} only considered single-antenna DUs while the proposed approach can naturally accommodates multi-antenna DUs.



\subsection{Our scheme - single DU} 
Now we describe our scheme.
First let us consider single DU case $M=1$. Recalling that our \emph{single} codeword is a $N^\text{tx}\times 1$ vector hence required number of bits does not depend on the number of transmit antennas, required number of bits for CU to transmit the $L\times 1$ data symbol vector $s$  to a single DU reads
\begin{align}
    B^\text{tot}_{\hat{x}} =  \underbrace{B_m}_{ \substack{ \text{ bits per} \\ \text{DU}} } \cdot \underbrace{N_\text{RB}\cdot 12\cdot14}_{\text{number of total data symbols}} \cdot \underbrace{2000}_{\text{number of slots per second}}.
\end{align}
Under same realizations in the previous subsection, we have $B_{\hat{x}}^\text{tot} = 0.092 \cdot B_m$ Gbps. Accordingly, for $25$ Gbps fronthaul capacity, we can use up to $B_m \leq 272.6$ bits/symbol. Comparison with benchmark scheme can be found in Fig.~\ref{fig:single_DU}.




\subsection{Benchmark that transmits precoding matrix and data symbols -- single DU}
{\color{blue} This subsection describes the conventional scheme with separate data/precoding compression, which will be implemented as a benchmark when studying SER/BER performance.}

Basic terminologies:
\begin{itemize}
    \item Resource block: $14$ OFDM time symbols ($=$ 1 slot) from $12$ subcarriers
    \item Bitwidth $B_W$ for precoding: quantization level for each element of $W$
    \item Bitwidth $B_s$ for data symbols: quantization level for each element of $s$ (logarithm of modulation order)
    \item Total number of resource blocks $N_\text{RB}$ in the wireless bandwidth ($N_\text{RB}=273$ for bandwidth $100$ MHz under subcarrier spacing $30$ kHz from 3GPP TS 38.104 [Table 5.3.2]).
    \item Number of resource blocks in frequency domain that \emph{share} the precoding matrix: $N_\text{RBG}$.
    \begin{itemize}
        \item Precoding matrix is fixed per slot; each slot uses different precoding
    \end{itemize} 
\end{itemize}

%Let us first denote quantization level per element in the precoding matrix (what they call as ``bitwidth'') as $B_W$, total number of resource blocks (each resource block is consisted of $14$ OFDM time symbols from $12$ subcarriers hence contains $168$ symbols) for data transmission as $N_\text{RB}$, number of resource blocks that \emph{share} the precoding matrix in frequency domain as $N_\text{RBG}$,   required number of bits for CU to transmit the $N^\text{tx} \times L$ precoding matrix $W$ to a single DU (per second) reads
Required number of bits for CU to transmit the $N^\text{tx} \times L$ precoding matrix $W$ to a single DU (per second) reads
\begin{align}
    B^\text{tot}_W = \underbrace{B_W \cdot N^\text{tx} \cdot L}_{\text{bits per precoding}} \cdot \underbrace{\frac{N_\text{RB}}{N_\text{RBG}}}_{\text{number of distinct precodings}} \cdot \underbrace{2000}_{\text{number of slots per second}}
\end{align}
while required number of bits for CU to transmit the $L\times 1$ data symbol vector $s$ to a single DU (per second) reads
\begin{align}
    B^\text{tot}_s =  \underbrace{B_s  \cdot L}_{ \substack{ \text{ bits per} \\ \text{data symbols}} } \cdot \underbrace{N_\text{RB}\cdot 12\cdot14}_{\text{number of total data symbols}} \cdot \underbrace{2000}_{\text{number of slots per second}}.
\end{align}
Assuming $N^\text{tx}=64, L=16, B_W=16, B_s=8, N_\text{RB}=273, N_\text{RBG}=4$, we have $B^\text{tot}_W = 2.24$ Gbps and $B_s^\text{tot} = 11.74$ Gbps ($2.24+11.74 < 25$). Illustration of single DU with $N^\text{tx}=64$ antennas can be found in Fig.~\ref{fig:single_DU}(a).






\section{Bo's comments on the fronthaul capacity}

\begin{figure}[h]
 %\begin{center}\includegraphics[scale=0.58]{Figs/seq.pdf}
 \begin{center}\includegraphics[scale=0.42]{Figs/single_du_co_distributed_antennas.pdf}
   \end{center}
   \caption{Massive MIMO implemented with single chip. In order to apply precoding, the chip needs to be equipped with $N^\text{tx}$ number of RF chains. (a) benchmark scheme that separately compresses data/precoding; (b) proposed scheme that directly compresses the precoded signal.} 
   \label{fig:single_DU}
\end{figure}


\begin{figure}[h]
 %\begin{center}\includegraphics[scale=0.58]{Figs/seq.pdf}
 \begin{center}\includegraphics[scale=0.37]{Figs/du_co_distributed_antennas.pdf}
   \end{center}
   \caption{Massive MIMO implemented with multiple chips. (left) $2$ chips each with $32$ RF chains, (middle) $4$ chips each with $16$ RF chains, (right) $8$ chips with $8$ RF chains; (top) single AAU case (co-located antennas), (b) multi-AAU case (distributed antennas) }
   \label{fig:multi_DU}
\end{figure}
\subsection{Multiple DUs -- multiple chips in single Active Antenna Unit (AAU)}

In order to adjust both amplitude and phase for every antenna element, we need one RF chain per single antenna element. Implementing a single chip as in Fig.~\ref{fig:single_DU} to contain all the required RF chains becomes demanding in massive MIMO scenarios. In this regard, as illustrated in Fig.~\ref{fig:multi_DU}(a)--(c), multiple \emph{cheap} chips each with fewer RF chains are implemented on behalf of single \emph{expensive} chip.

Noting that the total number of antennas $N^\text{tx}$ are fixed in this case ($N^\text{tx}=64$ for both Fig.~\ref{fig:single_DU} and Fig.~\ref{fig:multi_DU}), required number of bits for fronthaul link to transmit $N^\text{tx}/M \times L$ precoding matrix $W^{(m)}$ that corresponds to DU $m$ reads
\begin{align}
    B^\text{tot}_{W^{(m)}} = \underbrace{B_W \cdot \frac{N^\text{tx}}{M} \cdot L}_{\text{bits per precoding}} \cdot \underbrace{\frac{N_\text{RB}}{N_\text{RBG}}}_{\text{number of distinct precodings}} \cdot \underbrace{2000}_{\text{number of slots per second}}.
\end{align}
Accordingly, the benchmark scheme requires total number of bits $(B_{W^{(m)}}^\text{tot}+B_s^\text{tot})\cdot M = B_{W}^\text{tot}+B_s^\text{tot}\cdot M $ since each DU needs to receive entire data symbol vector $s$. This will easily exceed the $25$ Gbps since they want fronthaul capacity to remain as same as for single-DU case. On the other hand, as illustrated in Fig.~\ref{fig:du_proposed}, our scheme requires total number of bits $B_{\hat{x}}^\text{tot} \cdot M$, and assuming $64 $ DUs, we can use $B_m=4$ bits/symbol for each DU. We will investigate this by increasing the number of DUs.

\subsection{Multiple DUs -- multiple chips in multiple AAUs}
Next, we consider the case in which each DU corresponds to one single AAU, i.e., each DU has its own \emph{distributed} antennas as shown in Fig.~\ref{fig:multi_DU}(d)--(f). Note that difference between the case in the previous section (Fig.~\ref{fig:multi_DU}(a)--(c)) comes only from deployment of physical antenna elements (i.e., specification of the channel matrix $H$), hence analysis on the fronthaul capacity remains the same.


\begin{figure}[h]
 %\begin{center}\includegraphics[scale=0.58]{Figs/seq.pdf}
 \begin{center}\includegraphics[scale=0.48]{Figs/du_co_proposed.pdf}
   \end{center}
   \caption{Required number of bits for the fronthaul link when adopting the proposed framework: (a),(b) our scheme can save fronthaul capacity as compared to benchmark by compressing the precoded vector directly.}
   \label{fig:du_proposed}
\end{figure}

\subsection{Remarks}
They want fronthaul capacity to be linear in $N_\text{RB} \cdot N^\text{tx}$. We will check dependence of our scheme by considering the following experiments: (\emph{i}) fix $B_m$ to increase number of antennas; (\emph{ii}) scale $B_m$ with number of antennas, hoping that our $B_{\hat{x}}^\text{tot}$ grows linearly in $N_\text{RB}$ while (nearly) independent with $N^\text{tx}$ and $L$.


%On the other hand, since our scheme has its best improvement as compared to PtPQ  in few bits regime ($B_m < 6$), wondering we should play in the regime of many DUS $M \approx 50$ by n

Noting that we can use up to $B_m \cdot M \leq 272.6$ bits/symbol, we will check the performance of the proposed scheme by fixing $B_m \cdot M = 250$ and try out different combinations $(B_m,M)=(2,125), (5, 50), (10, 25), (25,10)$.. %Could you please share your thoughts on this? Thank you so much!

\newpage
\section{Plans on the experiments}
\begin{itemize}
    \item Common (new) terminologies: OFDM slot duration $T_\text{slot}$, number of OFDM symbols per slot $N_\text{OFDM}=14$, number of subcarriers per resource block $N_\text{SC}=12$, total number of RBs $N_\text{RB}$ 
    \item Terminologies for \emph{compression-precode} (CP) scheme: 
    number of RBs that share the precoding matrix $N^\text{CP}_\text{RBG}$, bitwidth for precoding $B_W$, bitwidth for data symbols $B_S$, required bits per second (bps) for CP scheme $B_\text{CP}$
    \item Terminologies for \emph{precode-compress} (PC) scheme: 
    number of RBs that share the codebook $N^\text{PC}_\text{RBG}$ (default $1$), bitwidth for precoded symbol $B_m$ per DU, required bits per second (bps) for CP scheme $B_\text{PC}$
    \item Basic setting: $N^\text{tx}=64, L=N^\text{rx}=16$ $(L_n=N_n^\text{rx}=2, N=8)$,  $N_\text{RB}=273$, $T_\text{slot}=0.5$ ms, 
    \begin{itemize}
        \item Basic settings for CP scheme: $N_\text{RBG}^\text{CP}=4$, $B_W=16$, $B_S=8$, $M \in \{1, 2, 4, 8, 16, 32, 64\}$ 
        \item This requires $14, 26, 50, 96, 190, 378, 753$ Gbps, for each $M$, respectively.
        \item Basic settings for PC scheme: $(B_m, M) \in \{ (150,1), (75, 2), (37, 4), (18, 8), (9, 16), (4,32), (2,64) \}$
        \item This requires $14$ Gbps
    \end{itemize}
    \item Assumption: CU knows perfect channel $H$ for each subcarrier and OFDM time symbol. 
    \item Study on the PC scheme under toy scenario (single carrier, $N=2$ single-antenna UEs, no comparison with CP scheme)
    \begin{itemize}
        \item ``sum-rate vs. number of training examples for codebook optimization'' (training and testing share the same channel statistics)  for $(B_m,M)\in \{(2, 5), (5, 2)\}$ given $N^\text{tx}_m=1$ ($\alpha$-PMQ assumes $\alpha=0.5$, $T=M$, unless specified otherwise)
        \item ``sum-rate vs. (parallel/total) computational complexity'' for $(B_m,M)\in \{(2, 5), (5, 2)\}$ given $N^\text{tx}_m=1$
        \item ``sum-rate vs. number of antennas $N_m^\text{tx}$'' fixing $B_m=2$
        \item ``sum-rate vs. number of antennas $N_m^\text{tx}$'' given $B_m=N_m^\text{tx}$
        \item ``sum-rate in the presence of channel estimation error vs. number of pilots $N_p$'' given total number of bits $B_p$ allocated for entire pilots
    \end{itemize}
    \item Realistic experiments (OFDM following the ``basic setting'' above)
    \begin{itemize}
        \item ``\emph{normalized} sum-rate vs. number of DUs $M$'' in which the normalized sum-rate is defined as $(\text{sum-rate}/B_\text{PC})$ for PC scheme and $(\text{sum-rate}/B_\text{CP})$ for CP scheme
        \item ``SER/BER vs. SNR'' with $\text{SNR}=P/\sigma^2$ (transmit power per DU $P$ divided by receiver noise variance $\sigma^2$)
        \item ``SER/BER vs. SNR'' in which the PC scheme suffers from mismatch in terms of parameters of the same channel model (Uma)
        \item ``SER/BER vs. SNR'' in which the PC scheme suffers from mismatch in terms of channel model (trained on Uma, testing on Umi)
        \item ``SER/BER vs. SNR'' in which the PC scheme shares the codebook across $N_\text{RBG}^\text{PC} \in \{1,2,4\}$ RBs
    \end{itemize}
\end{itemize}



==> Sections/B_experiments_before.tex <==


\newpage
\section{Comparison between CP and PC, Generalization Performance of Optimized Codebooks}
\subsection{Infinite Fronthaul Capacity}
We recall that per-DU power constraint, $\mathbb{E}[||\hat{x}_m||^2]\leq P$ for $m=1,...,M$, was taken into account during codebook optimization process. On the other hand, transmit vector with infinite fronthaul capacity $x=Ws$ may violate the per-DU power constraint depending on the choice of the precoding matrix $W$. In this report, we focus on the following \emph{fixed} normalized zero-forcing precoding to satisfy the looser \emph{total} power constraint $\mathbb{E}[||x||^2]\leq M\cdot P$. Accordingly, we define the normalized zero-forcing precoding matrix as 
\begin{align}
    \label{eq:precoding_power_const}
    W = \sqrt{\frac{M\cdot P}{\text{tr}(H^{-1} (H^{-1})^\dagger)}} H^{-1}
\end{align}
denoting $H^{-1}$ as the Moore–Penrose right pseudoinverse of matrix $H$. Defining precoding matrix as \eqref{eq:precoding_power_const}, total power constraint across all DUs can be directly satisfied as
\begin{align} \label{eq:power_contraint_W}
    \mathbb{E}[||x||^2] = \mathbb{E}[||Ws||^2] = \mathbb{E}[\text{tr}(Ws s^\dagger W^\dagger)] = \text{tr}(\mathbb{E}[W W^\dagger]) = M\cdot P.
\end{align}
The corresponding sum-rate for infinite fronthaul capacity can now be defined as
\begin{align}
    \sum_{n=1}^N \log_2\left(\frac{ \mathbb{E}_H[||H_n W_n||^2]+ \sigma^2 + \mathbb{E}_{H}[H_n K({x})H_n^\dagger]  }{\sigma^2 + \mathbb{E}_{H}[H_n K(x) H_n^\dagger ]}\right),
\end{align}
with $K(x)$ defined as the covariance matrix of the EI without quantization noise, i.e., $K(x)=\mathbb{E}_s[(x-W_ns_n)(x^\dagger-s_n^\dagger W_n^\dagger)]$. 

\subsection{Compress-precode (CP) scheme}
This subsection describes compress-precode (CP) scheme. As CP scheme shares a single precoding matrix for number $N_\text{SC}\cdot N_\text{RBG}$ of subcarriers across $N_\text{OFDM}$ time steps, corresponding precoding matrix $W^\text{CP}$ can be obtained by considering the \emph{average} channel matrix $\bar{H}$, i.e.,
\begin{align}
    \bar{H} = \frac{1}{N_\text{SC}\cdot N_\text{RBG} \cdot N_\text{OFDM}} \sum_{i=1}^{N_\text{OFDM}}\sum_{j=1}^{N_\text{SC}\cdot N_\text{RBG}} H_{i,j},
\end{align}
where we have denoted $H_{i,j}$ as the $N^\text{rx} \times N^\text{tx}$ channel matrix at time step $i$ and subcarrier index $j$. Taking $\bar{H}$ in lieu of $H$ in \eqref{eq:precoding_power_const}, precoding matrix for CP scheme $W^\text{CP}$ can be obtained. 

Given the precoding matrix $W^\text{CP}$, CP compresses each matrix element with $B_{W}$ number of bits via uniform quantization ($B_W/2$ for real and $B_W/2$ for imaginary part). We set the maximum and minimum value of the uniform quantizer based on $95\%$ confidence interval, i.e.., $[-1.96 \sigma_W,1.96 \sigma_W ]$, by approximately modelling each precoding element as Gaussian random variable with variance $\sigma_W^2 = M\cdot P/2N^\text{tx}\cdot L$ by noting that 
$\sum_{i=1}^{N^\text{tx}}\sum_{j=1}^{L}|W_{i,j}|^2 =||W||^2 = \text{tr}(W W^\dagger)= M\cdot P$ from \eqref{eq:power_contraint_W}  with $W_{i,j}$ the $(i,j)$ entry of matrix $W$. 






\subsection{Experimental Results}
We consider a distributed system with $M=4$ DUs and $N=4$ UEs. Each UE has  $N^\text{rx}_n=2$ antennas and wishes to receive $L_n=2$ symbols. All DUs are equpped with $N^\text{tx}_m=4$ antennas, either directional or omni-directional. More precisely, we assume that one of the $M$ DUs is located at the center of the cell, and has antennas directed towards the center of the sector, while the other DUs are randomly placed within the sector equipped with omni-directional antennas. 

\begin{figure}[t]
 \begin{center}\includegraphics[scale=0.28]{Figs/comp_CP_PC.pdf}
   \end{center}
   \caption{Sum-rate as a function of fronthaul capacity of PC schemes. CP schemes that adopt different quantization levels $B_W$ for precoding are also compared. For codebook optimization of PC schemes, we consider training and testing with same Uma channel, same large scale parameters, under same subcarrier.}
   \label{fig:comp_CP_PC}
\end{figure}
Recalling the definition of required number of bis per second (bps) for CP, $B_\text{CP}$, and required bps for the proposed precode-compress (PC) scheme, $B_\text{PC}$, we have the following ratio
\begin{align}
    \frac{B_\text{CP}}{B_\text{PC}} = \frac{L}{B_m}\cdot \left( \frac{B_W \cdot N^\text{tr}}{N_\text{RBG}\cdot N_\text{SC}\cdot N_\text{OFDM}} +B_S\right),
\end{align}
from which we can explicitly compute how much bps the proposed PC scheme can save as $B_\text{PC} = \frac{B_m}{0.05B_W + 64} \cdot B_\text{CP}$ under $N_\text{RBG}=4$. Since we consider continuous complex Gaussian symbol vector $s$, we set $B_S=8$ and assume that the symbol is perfectly transmitted for CP case. In Fig.~\ref{fig:comp_CP_PC}, we plot the sum-rate \eqref{eq:multi_antenna_sum_rate} as a function of the fronthaul capacity $B_m$ used by PC schemes. We compare with CP schemes under different number of bits $B_W\in\{4,8,16\}$ for precoding quantization. Even under $B_W=4$, PC schemes in Fig.~\ref{fig:comp_CP_PC} requires less than $10\%$ fraction of bps required by CP schemes, while achieving similar performance unless using extremely few $B_m \leq 2$ fronthaul capacity. Specifically, at $B_m=3$, PC schemes, especially the proposed ones -- tree-MQ and $\alpha$-PMQ -- use only $4.7\%$ bps of CP scheme ($B_W=4$) while achieving higher spectral efficiency. Similarly, under $B_m=4/B_m=5$, PC scheme uses $6.2\%/7.7\%$ bps of CP scheme ($B_W=8/B_W=16$), respectively, achieving similar spectral efficiency. 


\begin{figure}[t]
 \begin{center}\includegraphics[scale=0.34]{Figs/comp_topology.pdf}
   \end{center}
   \caption{Sum-rate as a function of fronthaul capacity of PC schemes. For codebook optimization of PC schemes, we consider training and testing with same Uma channel, same large scale parameters, under same subcarrier. Random codebooks are generated by uniform sampling from the $N_m^\text{tx}$-sphere with radius $\sqrt{P}$.}
   \label{fig:comp_random}
\end{figure}
Next, we focus on PC scheme to investigate the impact of codebook optimization by evaluating sum-rate of all PC schemes when equipped with random codebooks. We generate random codebook for each DU $m$ by uniformly sampling from the $N^\text{tx}_m$-sphere with radius $\sqrt{P}$. As shown in Fig.~\ref{fig:comp_random}, optimized codebooks always provide higher sum-rate as compared to random codebooks while the gap decreases with increased number of fronthaul capacity $B_m$ as similarly reported in \cite{lee2016multivariate}. Note that tree-MQ with random codebook cannot gain from increased fronthaul capacity since tree structure highly depends on the hierarchical codebook design that serves as resolution refinement which random codebook cannot provide. Random codebook design that takes into account for tree structure, e.g., split the sphere for random sampling at each depth, may be another interesting topic. 


\begin{figure}[h]
 \begin{center}\includegraphics[scale=0.34]{Figs/comp_random.pdf}
   \end{center}
   \caption{Sum-rate as a function of fronthaul capacity of PC schemes. For codebook optimization of PC schemes, we consider different discrepancies between training and testing: different subcarriers, different large scale parameters (topology), and different channel modellings (Uma/Umi).  Random codebooks are generated by uniform sampling from the $N_m^\text{tx}$-sphere with radius $\sqrt{P}$.}
   \label{fig:comp_gen}
\end{figure}

Lastly, we consider in Fig.~\ref{fig:comp_gen} the generalization performance of the proposed PC scheme for tree-MQ, $\alpha$-PMQ, and SMQ. First, we investigate whether PC schemes can generalize across different subcarriers by comparing different training appraoches for codebook: (\emph{i}) training codebook independently for each of the subcarrier, (\emph{ii}) training codebook jointly across different subcarriers.  Furthermore, generalization across different channel modellings are also considered by comparing (\emph{i}) training and testing both from Uma with fixed large scale parameters;   (\emph{ii}) training and testing both from Uma with different large scale parameters; and (\emph{iii}) training from Umi and testing for Uma. Surprisingly, Fig.~\ref{fig:comp_gen} shows that discrepancy between training and testing channel statistics yields negligible performance degradation, which may be understood by the following $t$-SNE visualization of the codebooks in Fig.~\ref{fig:tsne_carrier} and Fig.~\ref{fig:tsne_umi}. 


\begin{figure}[h]
 \begin{center}\includegraphics[scale=0.34]{Figs/vis_tsne.pdf}
   \end{center}
   \caption{$t$-SNE visualization of the codebooks. Each circle represents single codeword among codebook of size $2^{B_m}=4$ optimized per subcarrier, while different colors represent different subcarriers. Red crosses are for jointly optimized codebook that takes into account for $8$ different subcarriers. }
   \label{fig:tsne_carrier}
\end{figure}




In particular, Fig.~\ref{fig:tsne_carrier} compares codebooks with $2^B_m=2^2=4$ codewords, with $8$ different colors representing $8$ different subcarriers. Each colored circle in  Fig.~\ref{fig:tsne_carrier} represent a single codeword. In Fig.~\ref{fig:tsne_carrier} we also plot jointly optimized codebook that takes into account for all $8$ different subcarriers, hence plotted with red  crosses. Jointly optimized codewords and individually optimized codewords have similar representations in $t$-SNE plot hence explains the behavior of Fig.~\ref{fig:comp_gen}. Furthermore, Fig.~\ref{fig:tsne_umi} also depicts codebook optimized using different channel model, Umi, represented as black triangle markers. We can see that only one of the four codewords has different trend while the other three have similar representations with Uma codebook, which again validates that PC scheme is less vulnerable to overfitting. {\color{blue} In fact, I suspect my results.. I'm currently checking the channel models to see why we have such so small gap in quantitative (sum-rate) results. I think it would make more sense if for some case our scheme fails to generalize well.. maybe I can play with number of training examples for codebook optimization to see whether I'm making any mistakes... (currently each subcarrier has $100$ different small-scale fading realizations as training data. ) In the next version of the draft, I'll add results under channel estimation error (the U-shape) as well as SER/BER results...  }

\begin{figure}[h]
 \begin{center}\includegraphics[scale=0.34]{Figs/vis_tsne_umi.pdf}
   \end{center}
   \caption{ $t$-SNE visualization of the codebooks. Each circle represents single codeword among codebook of size $2^{B_m}=4$ optimized per subcarrier, while different colors represent different subcarriers. Black triangles are for codebook trained for different channel modelling -- Umi.}
   \label{fig:tsne_umi}
\end{figure}









\newpage







\section{Experimental Results}

In this section, we demonstrate the performance of tree-MQ and $\alpha$-PMQ via comparisons with SMQ \cite{lee2016multivariate} and with point-to-point quantization (PtPQ). MQ is not implemented due to the excessive computation load. In PtPQ, quantization takes place independently per node by solving the problem $\min_{\hat{x} \in \hat{\mathcal{X}}_{m}}||\hat{x} - x_m||$ for each DU $m$. Given the quantized vector, the codebook optimization follows problem  \eqref{eq:obj_wonju_codebook}.

For the numerical study in this section, we assume that each DU has $N_m^\text{tx}=4$ antennas {\color{blue} and that they follow 3GPP urban macrocell (UMa) channel modelling}. We adopt zero-forcing precoding. %and that there are $N=10$ single-antenna UEs. {\color{blue} We will consider multi-antenna UEs in the next subsection}. We assume 3GPP urban macrocell (UMa) setting to model the channel matrix $H$. We adopt zero-forcing precoding.


% \begin{figure}[h]
%   \begin{center}\includegraphics[scale=0.46]{Figs/sys_uma.pdf}
%     \end{center}
%     \caption{Assumed communication environment in a single cell: Each DU is equipped with $N_m^\text{tx}=4$ antennas to serve $N=10$ single-antenna UEs. (a) $M=4$ DUs with fronthaul capacity $B_m=3$ bits per symbol; (b) $M=6$ DUs with fronthaul capacity $B_m=2$ bits per symbol. 3GPP urban macrocell (UMa) \cite{3gpp} is assumed for channel modelling.}
%     \label{fig:sys_experiment_uma}
%  \end{figure}
 
 
 \begin{figure}[h]
  \begin{center}\includegraphics[scale=0.18]{Figs/M_6_single.png}
    \end{center}
    \caption{Spectral efficiency as a function of (top) normalized total computational complexity (bottom) normallized parallel computational complexity. We assume  $M=6$ DUs equipped with $N_m^\text{tx}=4$ antennas under fronthaul capacity $B_m=2$ and $N=10$ single-antenna UEs. Reported values are averaged over $100$ different channel realizations with $100$ different symbols per channel realization. For both training and testing, the same, fixed, large scale parameters \cite{3gpp} of DUs and UEs are assumed. }
    \label{fig:results_tree_and_pmq}
 \end{figure}

  
 \begin{figure}[h]
  \begin{center}\includegraphics[scale=0.18]{Figs/M_4_single.png}
    \end{center}
    \caption{Spectral efficiency as a function of (top) normalized total computational complexity (bottom) normallized parallel computational complexity. We assume  $M=4$ DUs equipped with $N_m^\text{tx}=4$ antennas under fronthaul capacity $B_m=3$ and $N=10$ single-antenna UEs. Reported values are averaged over $100$ different channel realizations with $100$ different symbols per channel realization. For both training and testing, the same, fixed, large scale parameters \cite{3gpp} of DUs and UEs are assumed. }
    \label{fig:results_tree_and_pmq_2}
 \end{figure}
 
 


In order to optimize the codebook, for all schemes, we assume the availability of $100$ different channel realizations with $100$ different symbols per channel realization, and the symbols for each UE are generated by complex standard normal distribution $\mathcal{CN}(0,1)$ as in \cite{lee2016multivariate}. We set the average signal-to-noise ratio (SNR) for each DU as $P/\sigma^2=10 \text{ dB}$.

We are interested in studying spectral efficiency versus computational complexity. We consider two metrics: (\emph{i}) \emph{total number of operation}, with one operation unit corresponding to the evaluation of the EI in \eqref{eq:EI_multi_antenna}; and (\emph{ii}) \emph{number of operations on a parallel processor}, whereby parallel operation at different subprocessors are counted only once. The table below reviews the complexity measures for all schemes assuming $B_m=B$ for all DUs $m=1,...,M$. In the table, we evaluate total computational complexity of $\alpha$-PMQ by defining the number of iterations as $T$ and the average number of DUs included in an iteration as $M'$.   We plot performance as a function of complexity normalized by the complexity of PtPQ. 


\begin{table}
  \caption{Computational complexity in terms of total number of operation and number of operations on a parallel processor ($T$ is the number of iterations of $\alpha$-PMQ and $M' \leq M$ is the average number of DUs included in each step)}
  \label{table:tab_comp_comp}
  \centering
  \begin{tabular}{l|l|l}
    scheme & total & parallel \\ 
    \midrule
    PtPQ & $M \cdot 2^B$  & $2^B$     \\
    MQ     & $2^{MB}$ & $2^{MB}$      \\
    SMQ     & $M\cdot 2^B$      & $M\cdot 2^B$ \\
    tree-MQ     & $B\cdot 2^M$      &  $B\cdot 2^M$ \\
    $\alpha$-PMQ     & $T \cdot M'\cdot 2^B$      & $T\cdot 2^B$  \\
  \end{tabular}
\end{table}


\subsection{Single-Antenna UE}
{\color{blue}First, we assume $N=10$ single antenna UEs hence $L_n=1$ transmit symbol per each UE.} In Fig.~\ref{fig:results_tree_and_pmq}, we consider $M=6$ DUs with fronthaul capacity $B_m=2$, and in Fig.~\ref{fig:results_tree_and_pmq_2} we consider $M=4$ DUs with fronthaul capacity $B_m=3$. We set $\alpha=0.5$ for $\alpha$-PMQ, and we vary the complexity of $\alpha$-PMQ by increasing the number $T$ of iteration. Accordingly, all schemes but $\alpha$-PMQ provide a single point in the performance-complexity trade-off. 

Tree-MQ outperforms SMQ \cite{lee2016multivariate} at the cost of a larger computational complexity. $\alpha$-PMQ outperforms both tree-MQ and SMQ in terms of spectral efficiency. Furthermore, in the presence of a parallel processor, the performance improvement is obtained at a lower computational complexity. Specifically, with a parallel processor, for a fixed spectral efficiency, $\alpha$-PMQ has lowest computational complexity; while for a fixed computational complexity, $\alpha$-PMQ has the highest spectral efficiency.


The spectral efficiency benefits of $\alpha$-PMQ hinge on the possibility to isolate the groups of DUs with limited mutual interference. Accordingly, for more complex systems, such as that considered in Fig.~\ref{fig:results_tree_and_pmq} as compared to Fig.~\ref{fig:results_tree_and_pmq_2}, $\alpha$-PMQ exhibits the largest performance gains. Furthermore, as discussed, the computational complexity savings of $\alpha$-PMQ are realized when  allowing for parallel computations across multiple DUs, i.e., $M'=1.88$ for Fig.~\ref{fig:results_tree_and_pmq}, and $M'=1.68$ for Fig.~\ref{fig:results_tree_and_pmq_2}.



\begin{figure}[h]
  \begin{center}\includegraphics[scale=0.213]{Figs/M_6_multi.png}
    \end{center}
    \caption{Spectral efficiency as a function of (left) normalized total computational complexity (right) normallized parallel computational complexity. We assume  $M=6$ DUs equipped with $N_m^\text{tx}=4$ antennas under fronthaul capacity $B_m=2$ and $N=5$ multi-antenna UEs ($N_n^\text{rx}=2)$ as well as single-antenna UEs. Reported values are averaged over $100$ different channel realizations with $100$ different symbols per channel realization. For both training and testing, the same, fixed, large scale parameters \cite{3gpp} of DUs and UEs are assumed. }
    \label{fig:multi_M_6}
 \end{figure}

  
 \begin{figure}[h]
  \begin{center}\includegraphics[scale=0.213]{Figs/M_4_multi.png}
    \end{center}
    \caption{Spectral efficiency as a function of (left) normalized total computational complexity (right) normallized parallel computational complexity. We assume  $M=4$ DUs equipped with $N_m^\text{tx}=4$ antennas under fronthaul capacity $B_m=3$ and $N=5$ multi-antenna UEs ($N_n^\text{rx}=2)$ as well as single-antenna UEs. Reported values are averaged over $100$ different channel realizations with $100$ different symbols per channel realization. For both training and testing, the same, fixed, large scale parameters \cite{3gpp} of DUs and UEs are assumed. }
    \label{fig:multi_M_4}
 \end{figure}
 
{\color{blue} \subsection{Multi-Antenna UE}}
Next, in Fig.~\ref{fig:multi_M_6} and Fig.~\ref{fig:multi_M_4}, we consider a system with $N=5$ multi-antenna UEs equipped with $N_n^\text{rx}=2$ antennas that aims at receiving $L_n=2$ complex symbols.  Other settings are same as in the previous section, i.e., Fig.~\ref{fig:multi_M_6} and Fig.~\ref{fig:multi_M_4} follow the same setting as Fig.~\ref{fig:results_tree_and_pmq} and Fig.~\ref{fig:results_tree_and_pmq_2}, respectively. Furthermore, to clarify the impact of the increased number of antennas of UE, comparison with $N=5$ single-antenna UEs is also made in Fig.~\ref{fig:multi_M_6} and Fig.~\ref{fig:multi_M_4}.

While general trends follow the same as in the previous subsection, we can clearly see that UEs equipped with multiple antennas clearly achieve higher spectral efficiency as compared to single-antenna UEs.
 

\subsection{Channel Estimation Error}
Now we investigate the impact of channel estimation noise by evaluating the spectral efficiency as described in \eqref{eq:multi_antenna_sum_rate_ch_est}. Pilot symbols are generated by sampling from complex standard normal distribution $\mathcal{CN}(0,1)$ in a same manner with data symbols.  
$M=2$ DUs with fronthaul capacity $B_m=2$ and $N=2$ multi-antenna UEs ($N_n^\text{rx}=2$, $L_n=2$) are assumed. 
In Fig.~\ref{fig:ch_est}, dashed line represents spectral efficiency without channel estimation noise while solid line depicts spectral efficiency with channel estimation noise. We plot the figure as a function of number of pilots $N_p$. Unlike conventional system, as pilots also suffer from quantization noise, increased number of pilots does not necessarily improve the spectral efficiency. 

Fig.~\ref{fig:ch_est_2} has the same setting as Fig.~\ref{fig:ch_est} assuming single-antenna UEs. We can see from Fig.~\ref{fig:ch_est_2} that in some cases, increased number of pilots can be beneficial since it decreases the last term of channel estimation error $E_n$ (see \eqref{eq:hat_H_n}). 

{\color{blue} I was trying to do some experiments that we can clearly investigate both terms of $E_n$. In particular, I was expecting that under high fronthaul capacity, the spectral efficiency would go up as the number of pilots increases. But it still decreases with $B_m=7$.. I think the reason comes from discrepancy between $\hat{x}$ and $W s$  even under infinite capacity due to the power constraint. Maybe I should have designed precoding matrix (via normalizing) so that even $W s$ satisfies the power constraint... Could you please share your thoughts on this?}

  
 \begin{figure}[h]
\begin{center}\includegraphics[scale=0.213]{Figs/ch_est.png}
    \end{center}
    \caption{Spectral efficiency as a function of number of pilots $N_p$. We assume  $M=2$ DUs equipped with $N_m^\text{tx}=4$ antennas under fronthaul capacity $B_m=2$ and $N=2$ multi-antenna UEs ($N_n^\text{rx}=2)$. Dashed line assumes perfect channel estimation while solid line takes into account for channel estimation noise from $N_p$ pilots. Reported values are averaged over $100$ different channel realizations with $100$ different symbols per channel realization. For both training and testing, the same, fixed, large scale parameters \cite{3gpp} of DUs and UEs are assumed. }
    \label{fig:ch_est}
 \end{figure}
 


 \begin{figure}[h]
\begin{center}\includegraphics[scale=0.213]{Figs/ch_est_2.png}
    \end{center}
    \caption{Spectral efficiency as a function of number of pilots $N_p$. We assume  $M=2$ DUs equipped with $N_m^\text{tx}=4$ antennas under fronthaul capacity $B_m=2$ and $N=2$ single-antenna UEs ($N_n^\text{rx}=1)$. Dashed line assumes perfect channel estimation while solid line takes into account for channel estimation noise from $N_p$ pilots. Reported values are averaged over $100$ different channel realizations with $100$ different symbols per channel realization. For both training and testing, the same, fixed, large scale parameters \cite{3gpp} of DUs and UEs are assumed. }
    \label{fig:ch_est_2}
 \end{figure}
 


==> Sections/WMMSE.tex <==
\begin{algorithm}[t!] \label{alg:alpha_pmq}
    \caption{WMMSE Precoding Design}
    \SetKwInOut{Input}{Input}
    \Input{channel matrix $H$; noise variance $\sigma^2$; power constraints $P_m$ for RU $m=1,...,M$; convergence threshold for sum-rate $R^\text{th}$, convergence threshold for power $P^\text{th}$; maximum iteration $I$}
    \SetKwInOut{Output}{Output}
    \Output{precoding matrix $W$}
    \textbf{Initialize} precoding matrix $W$; sum rate $R^\text{prev} \leftarrow 0$\\
    \For{\emph{$i=1,...,I$}}{
        calculate receiver beamforming matrix
        \begin{align}
            F_n = \Big( \sum_{n'=1}^N H_n W_{n'}W_{n'}^\dagger H_n^\dagger + \sigma^2 I \Big)^{-1} H_n W_n. \nonumber 
        \end{align}
        calculate sum-rate
        \begin{align}
            R = \sum_{n=1}^N \log \big| I + J_n^{-1} H_n W_n W_n^\dagger H_n^\dagger \big|, \nonumber 
        \end{align}
        with $J_n = \sum_{n'=1, n' \neq n}^{N} H_n F_{n'} F_{n'}^\dagger H_n^\dagger + \sigma^2 I$ \\
        \uIf{$|R - R^\text{prev}| < R^\text{th}$}{
         break
          }
        $R^\text{prev} \leftarrow R$\\ 
        calculate the weight matrix
        \begin{align}
            \Theta_n = \Big( (F_n^\dagger H_n W_n - I)(F_n^\dagger H_n W_n - I)^\dagger + \sum_{n'=1, n'\neq n}^N F_n^\dagger H_n W_{n'} W_{n'}^\dagger H_n F_n + \sigma^2 F_n^\dagger F_n \Big)^{-1} \nonumber 
        \end{align}
        calculate required matrices for precoding update
        \begin{align}
            &A_n = H_n^\dagger F_n \Theta_n F_n^\dagger H_n; \quad A_n = A_n^{1/2}(A_n^{1/2})^\dagger \nonumber\\
            &A_n^{1/2} = [\hat{A}_{1,n}^\dagger, ..., \hat{A}_{M,n}^\dagger]^\dagger; \quad
            \tilde{A}_{m,n} = \hat{A}_{m,n}\sum_{m'=1, m'\neq m}^M \hat{A}_{m',n}^\dagger W_{m', n} \nonumber 
        \end{align}
        \For{\emph{$m = 1,...,M$}}{
        update precoding matrix for RU $m$ as
        \begin{align} 
        W_{m,n}(\mu_m) = (Q_{m,n}+\mu_m I)^{-1} M_{m,n},\nonumber 
        \end{align}
        with $M_{m,n} = C_{m,n} - \tilde{A}_{m,n}, Q_{m,n} = \hat{A}_{m,n}\hat{A}_{m,n}^\dagger$ given $C_n = H_n^\dagger F_n \Theta_n = [C_{1,n}^\dagger, ..., C_{M,n}^\dagger]^\dagger$, while setting the power $\mu_m$ via bisection to ensure $|\text{tr}(W_{m,n}^\dagger(\mu_m)W_{m,n}(\mu_m)) - P_m| \leq P^\text{th}$ \\
    }
    }
    \textbf{Return} $W$
    \end{algorithm}
  


==> Sections/backup_3_b_EI_tmp.tex <==
{\color{blue}
\section{Computational Analysis and Preliminary Results for Channel Estimation} \label{sec:detailed_comp_complexity}
In this section, we compare the computational complexity of CP and PC in terms of number of floating point operations (flops). Since CP and PC have different functional split as described throughout the paper, we will make the comparison at the DU and RU side separately. In order to provide explicit flops formula, we first describe the simple  MMSE precoding design adopted in this work. 

%with $N_n^\text{rx}\times N^\text{tx}$ per-UE channel matrix $H_n$ for UE $n$,

\subsection{MMSE Precoding Design}
Given the $N^\text{rx} \times N^\text{tx}$ full channel matrix $H = [H_1^\dagger,...,H_N^\dagger]^\dagger$, we first reduce the dimension of row space of $H_n$ from $N_n^\text{rx}$ to $L_n$ by projecting $H_n$ to the reduced eigenspace of $H_n H_n^\dagger$ defined via $L_n$ eigenvectors with $L_n$-largest singular values, i.e., obtain dimension-reduced matrix $\tilde{H}_n$ as 
\begin{align}
    \tilde{H}_n = U_{:, 1:L_n}^\dagger H_n, 
\end{align}
denoting as $U_{:, 1:L_n}$ the collection of the first $L_n$ columns of $U_n$ given $H_n = U_n \Sigma_n V_n^\dagger$. We assume that singular values in $\Sigma_n$ are sorted in a descending order. Then we can obtain standard MMSE precoding matrix $W$ given $\tilde{H} = [\tilde{H}_1^\dagger, ..., \tilde{H}_N^\dagger]^\dagger$ along with power scaling factor $r_m$ for RU $m$ as
\begin{align}
    W = \text{diag}(r_1,...,r_M) \cdot \tilde{H}^\dagger (\tilde{H}\tilde{H}^\dagger + \xi I)^{-1},
\end{align}
given the regularization factor $\xi = N^\text{rx}/\sum_{m=1}^M P_m$ \cite{schmidt2008minimum}. Then, denoting as $\tilde{W} = \tilde{H}^\dagger (\tilde{H}\tilde{H}^\dagger + \xi I)^{-1} $ the unnormalized precoding matrix, the power scaling factor $r_m$ can be obtained as 
\begin{align}
    r_m = \sqrt{\frac{P_m}{\text{tr}(\tilde{W}_m^\dagger \tilde{W}_m)}}, 
\end{align}
denoting as $\tilde{W}_m$ the unnormalized precoding matrix associated to RU $m$. Related computational complexity analysis can be found in Table~\ref{table:tab_comp_comp_DU} and Table~\ref{table:tab_comp_comp_RU} that also encompass the complexities of  both CP and the proposed neural-MQ.



\begin{table} \hspace{-1.5cm}
\begin{threeparttable}
  \caption{Computational complexity at DU per channel use}
  \label{table:tab_comp_comp_DU}
  \centering
  \begin{tabular}{l|l|l}
    operation & flops formula  & value \\ 
    %\midrule
    \hline
    \hline
    SVD of $H_n=U_n \Sigma_n V_n^\dagger$ for $n=1,...,N$ &  $(2N^\text{tx}(N_n^\text{rx})^2 + 11(N_n^\text{rx})^3) \cdot N$ & $44,032$    \\
    \hline
    \begin{tabular}[x]{@{}c@{}}dimension reduction $\tilde{H}_n = (U_{:, 1:L_n})^\dagger H_n $ for $n=1,...,N$\\($U_{:,1:L_n}$ is the collection of the first $L_n$ columns of $U_n$\end{tabular} &   $(2 L_n N_n^\text{rx} N^\text{tx})\cdot N$  & $8,192$   \\
    \hline
    $\tilde{H}\tilde{H}^\dagger (\tilde{H} = [\tilde{H}_1^\dagger,...,\tilde{H}_n^\dagger ]^\dagger)$ &  $2 L^2 N^\text{tx}$  & $32,768$     \\
    \hline
    $(\tilde{H}\tilde{H}^\dagger + \xi I)^{-1}$ &  $2 L^3/3$  & $2,731$ \\
    \hline
    $\tilde{W} = \tilde{H}^\dagger \cdot (\tilde{H}\tilde{H}^\dagger + \xi I)^{-1}$ &  $2 N^\text{tx} L^2$  & $32,768$  \\
    \hline
    power scaling $r_m= \sqrt{P_m/\text{tr}(\tilde{W}_m^\dagger \tilde{W}_m)}$ for $m=1,...,M$ &  $(2\cdot \min{(L^2 N_m^\text{tx}, (N_m^\text{tx})^2 L)})\cdot M$  & $32,768$    \\
    \hline 
    \begin{tabular}[x]{@{}l@{}} neural-MQ with one hidden layer with  number of \\ hidden neurons $N_\text{net}$ for  $m=1,...,M$: $I$ GD steps\end{tabular} 
     &  $\Big(I \cdot \big( 2 \cdot 2\cdot ( B_m N_\text{net}+2N_\text{net}N_m^\text{tx})/3 + 2N^\text{rx}(N^\text{tx} + L_n) + 3 L \big) \Big)\cdot M$   & \begin{tabular}[x]{@{}c@{}} $66,240 \cdot I$ for $N_\text{net}=64$\\
     $43,712 \cdot I$ for $N_\text{net}=20$ \\
     $38,592 \cdot I$ for $N_\text{net}=10$ \\ $36,032 \cdot I$ for $N_\text{net}=5$\end{tabular}    \\
    % \hline
    % \begin{tabular}[x]{@{}l@{}} neural-MQ without hidden layer $K=0$ for  $m=1,...,M$: \\ $I$ GD steps\end{tabular} 
    %  &  $\Big(I \cdot \big( 2 \cdot 2\cdot (2B_mN_m^\text{tx})/3 + 2N^\text{rx}(N^\text{tx} + L_n) + 3 L  \big) \Big)\cdot M$   & $10,923 \cdot I$    \\   
  \hline
  \hline
  \end{tabular} 
  \begin{tablenotes}
      \small
      \item First $6$ lines are related to MMSE precoding matrix design per channel use. Last line corresponds to the proposed neural-MQ per channel use. Computational complexity of precoding matrix design can be reduced when one shares precoding matrix across multiple channel uses. We assume $M=4$ DUs and $N=16$ UEs, each equipped with $N_m^\text{tx}=16$ transmit antennas and $N^\text{rx}=4$ receive antennas, in which each UE wishes to receive $L_n=1$ data stream. 
    \end{tablenotes}
  \end{threeparttable}
\end{table}


\begin{table}
\begin{threeparttable}
  \caption{Computational complexity at RU per channel use}
  \label{table:tab_comp_comp_RU}
  \centering
  \begin{tabular}{l|l|l}
    operation & flops formula  & value   \\ 
    \midrule
    weight application $x=W s$ with $W=\text{diag}(r_1,...,r_M)\tilde{W}$&  $2 N^\text{tx} L$   & $2,048$    \\
    \hline
    neural-MQ  for $m=1,...,M$: one inference&  $  (2\cdot (B_mN_\text{net}+2N_\text{net}N_m^\text{tx})/3)\cdot M$  &  
    \begin{tabular}[x]{@{}c@{}} 
    $16,384$ for $N_\text{net}=64$\\
    $5,120$ for $N_\text{net}=20$\\ $2,560$ for $N_\text{net}=10$\\ $1,280$ for $N_\text{net}=5$\end{tabular} 
    \\
  \end{tabular}
  \begin{tablenotes}
      \small
      \item First line corresponds to precoding matrix application for CP. Second line corresponds to neural codebook application for PC.  We assume $M=4$ DUs and $N=16$ UEs, each equipped with $N_m^\text{tx}=16$ transmit antennas and $N^\text{rx}=4$ receive antennas, in which each UE wishes to receive $L_n=1$ data stream. 
    \end{tablenotes}
  \end{threeparttable}
\end{table}


}


\subsubsection{Channel Estimation based on DMRS} We consider DMRS configuration type $1$ that can deal with $8$ orthogonal channel estimation, recalling that we have total number of streams $L = N\cdot L_n = 8$. Given the estimated pilot channel obtained via least squares estimate, we then apply MMSE interpolation \cite{hoeher1997two} to obtain channel estimate for the payload data. Channel statistics for MMSE interpolation is obtained by assuming that multipath components are uniformly distributed in time domain within the upper bound of the delay spread \cite{3gpp}, assuming $95\%$ confidence level. Total power across the multipath components are set to $1$ as we consider normalized channel realization for the experiment. 

In Fig.~\ref{fig:pilot_dmrs} below, we show some preliminary results in the presence of channel estimation error. We plot both the sum spectral efficiency as well as the averaged symbol error rate as a function of fronthaul capacity $B^\text{pilot}$ assumed by DMRS pilot symbols. We set $B_m=64$ for PC, while PC and CP assume precoding sharing across $12\cdot 14$ channel uses (1 RB), hence MMSE interpolation is done within this 1 RB. Note that CP does not require additional fronthaul overhead for pilot transmission. For PC, quantization of the pilot symbols are done via neural-PtPQ by noting that the pilot symbols are designed to be orthogonal across different UEs. We can see that neural-MQ still outperforms CP in the presence of channel estimation error. 








\begin{figure}[h]
  \begin{center}\includegraphics[scale=0.4]{Figs/dmrs.pdf}
    \end{center}
    \caption{Sum spectral efficiency (left) and averaged symbol error rate (right) as a function of fronthaul capacity $B^\text{pilot}$ assumed by DMRS symbols. We set fronthaul capacity for payload data to $B_m=64$. We assume $M=4$ RUs equipped with $N_m^\text{tx}=16$ antennas and $N=4$ multi-antenna UEs equipped with $N_n^\text{rx}=4$ antennas that wishes to receive $L_n=2$ independent data streams. The reported values are averaged over $5$ different channel realizations with $10000$ different symbols, while optimization uses $100$ channels and $100$ symbols. The positions of the RUs are fixed, while UE positions are randomly distributed for each channel realization. The channel is generated by following 3GPP urban micro (UMi) modelling \cite{3gpp}. }
    \label{fig:pilot_dmrs}
 \end{figure}



\newpage


% \subsection{Exact Gradient Expression}
% In this subsection, we analyze the computational complexity of the proposed gradient-based neural-MQ (\ref{eq:gradient_based_quan}) by explicitly writing down the gradient in terms of basic operations such as matrix multiplication. Let us first denote as $A_k = \text{diag}(A_{1,k},...,A_{M,K})$ and $c_k = [c_{1,k}^\top,...,c_{M,k}^\top]^\top$  the collection of weight matrices and biases vectors from $M$ RUs at the $k$-th (hidden) layer, i.e., $\theta_m = \{A_{m,k}, c_{m,k}\}_{k=1}^K$ and $\theta_{1:M} = \{ A_k, c_k \}_{k=1}^K$, with which  the output of the $k$-th layer $\tilde{x}_{k}$ can be determined as $\tilde{x}_{k} = g_k(A_k \tilde{x}_{k-1} + c_{k})$ given some activation function $g_k(\cdot)$ at layer $k$, with  $\tilde{x}_0 = \sigma_\tau(r_{1:M})$ and $\tilde{x}_K = \hat{x}$. We particularly consider ELU activation for $g_{k}(\cdot)=\color{blue}{..}$ for $k < K$ and identity mapping for $g_K(\cdot)$. Finally, denoting $\text{C2R}(\cdot)$ as a reshaping function that maps a complex vector $\mathbb{C}^{N^\text{tx}}$ to a real vector $\mathbb{R}^{2N^\text{tx}}$ by taking real and imaginary component separately, the gradient in (\ref{eq:gradient_neural_MQ}) can be explicity written as 
% \begin{align} \label{eq:gradient_neural_MQ}
%     &\nabla_{r_{1:M}} \sum_{n=1}^N \text{EI}_n(x, f(\sigma_\tau(r_{1:M})|\theta_{1:M})  ) \nonumber\\&= \text{diag}\bigg( \frac{e^{-r_{1:M}/\tau}}{\tau \cdot (1+ e^{-r_{1:M}/\tau} )^2} \bigg)\cdot \prod_{k=1}^K  A_{k}^\top \text{diag}\Big( \text{ReLU}(A_k \tilde{x}_k + c_k) + \text{ReLU}(-A_k \tilde{x}_k - c_k)e^{A_k \tilde{x}_k + c_k}\Big) \nonumber\\
%     &\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\cdot \text{C2R}\bigg( \sum_{n=1}^N \Big( 2\text{Re}( G_n^\dagger(G_n \tilde{x}_{K} - s_n)  ) \Big) \bigg)
% \end{align}

% which requires computatational complexity ... diagonal... parallel across M ... 


%A_{k}^\top \text{diag}\bigg( \text{ReLU}(A_k \tilde{x}_k + c_k) + \text{ReLU}(-A_k \tilde{x}_k - c_k)e^{}\bigg)

% \begin{align}
%     \label{eq:obj_neural_codebook}
%     \min_{ \{f_m(\cdot)\}_{m=1}^M } \mathbbm{E}\bigg[ \sum_{n=1}^N \text{EI}_n(\hat{x}) \bigg]& \nonumber\\
%     \text{s.t. } (\ref{eq:neural_MQ_overall}),&
% \end{align}






% However, as constrained optimization for neural network is often a challenging task unlike constrained convex optimization problem, we instead train the neural network in an \emph{unconstrained} manner, then to impose the average power constraint in a \emph{post-hoc manner}, which will be specified in the next subsection. Accordingly, training the neural codebook $f_m(\cdot)$ can be simply done by solving
% \begin{align}
%     \label{eq:neural_codebook_opt}
%     &\min_{  \{f_m(\cdot)\}_{m=1}^M  } \mathbbm{E}_{H,s}\bigg[ \sum_{n=1}^N  \text{EI}_n(  f(b_{1:M})  ) \bigg] \nonumber\\
%     &\text{ s.t. }  b_{1:M} = \texttt{neural-MQ}(s, H, W, F|f_1,...,f_M),
% \end{align}
% where the expectation is approximated with available channel realizations and symbol realizations. In the following section, we will show how we impose average power constraint during neural-MQ process hence, to modify the optimization (\ref{eq:neural_codebook_opt}) accordingly.


% \subsection{Achieving Average Power Constraint via Self-Normalization}
% Training the neural codebooks $\{f_m(\cdot)\}_{m=1}^M$  via  (\ref{eq:neural_codebook_opt}) does not guarantee the average power constraint (\ref{eq:avg_power_constraint}). In order to satisfy the condition (\ref{eq:avg_power_constraint}) for each channel realization $H$, we consider \emph{joint optimization} across multiple $K$ channel uses during the channel coherence time, and impose the average power constraint across the $K$ channel uses. To begin with, let us denote $b_{1:M}^k$ as the binary vectors for $M$ RUs obtained by neural-MQ given symbol $s^k$ at channel use $k$. The $K$ binary vectors $ b^1_{1:M},...,b^K_{1:M}$ across $K$ channel uses can be jointly obtained by solving
% \begin{align} \label{eq:N_MQ_obj_joint}
%     b^1_{1:M},...,b^K_{1:M} &= \arg\min_{b^1_{1:M}, ..., b^K_{1:M} }  \sum_{k=1}^K \sum_{n=1}^N \text{EI}_n( [(\hat{x}_1^k)^\top,...,(\hat{x}_M^k)^\top]^\top ),\nonumber\\
%     &\text{ s.t. } \hat{x}_m^k = \sqrt{\frac{K\cdot P_m}{\sum_{k'=1}^K || f_m( b^{k'}_{m}) ||^2}} \cdot f_m(   b^k_{m}    ) \text{ for all } m=1,...,M
% \end{align}
% which can be solved via gradient-based approach as done in (\ref{eq:gradient_based_quan}). Note that in (\ref{eq:N_MQ_obj_joint}),  the transmit vector $\hat{x}^k_m$ for each RU $m$ at channel use $k$ is \emph{self-normalized}, which guarantees the average power constraint across $K$ channel uses, i.e., 
% \begin{align}
% \frac{1}{K}\sum_{k=1}^K || \hat{x}_m^k ||^2 = P_m.    
% \end{align}
% Algorithm~\ref{alg:joint_neural_MQ} summarizes the joint neural-MQ procedure, and we have denoted $[\hat{x}_m]_{m=1}^M$ as $\hat{x}$, i.e., $[\hat{x}_m]_{m=1}^M= [\hat{x}^\top_1,...,\hat{x}^\top_M]^\top$.

% Assuming such joint optimization of neural-MQ, the optimization procedure of neural codebook can be as well modified by taking joint neural-MQ process in Algorithm~\ref{alg:joint_neural_MQ} in lieu of \texttt{neural-MQ}$(s,H,W,F|f_1,...,f_M)$ in (\ref{eq:neural_codebook_opt}). More precisely, denoting  \texttt{neural-MQ}$(s^{1:K},H,W,F|f_1,...,f_M)$ as the algorithmic function that corresponds to Algorithm~\ref{alg:joint_neural_MQ}, the neural codebooks can be optimized by solving
% \begin{align}
%     \label{eq:joint_neural_codebook_opt}
%     &\min_{  \{f_m(\cdot)\}_{m=1}^M  } \mathbbm{E}_{H,s}\bigg[ \sum_{k=1}^K \sum_{n=1}^N  \text{EI}_n\bigg( \bigg[  \sqrt{\frac{K\cdot P_m}{\sum_{k'=1}^K || f_m( b^{k'}_{m}) ||^2}} \cdot f_m(   b^k_{m}    )  \bigg]_{m=1}^M \bigg) \bigg] \nonumber\\
%     &\text{ s.t. }  b^1_{1:M},...,b^K_{1:M} = \texttt{neural-MQ}(s^{1:K}, H, W, F|f_1,...,f_M).
% \end{align}








% \subsection{Infinite Fronthaul Benchmark}

% {\color{blue} Surprisingly, neural-MQ without binary constraint (without temperature anealing to send $\tilde{b}_{1:M}$ directly using infinite fronthaul) was outperformed by neural-MQ. I suspect this is somehow related to generalization analysis but let me figure this out shortly so that we can have proper, tighter, upper bound for our neural-MQ .. }

% Given infinite fronthaul capacity, DU can losslessly transmit the precoded vector $x_m = W_{m,:} s$ to each RU $m$. However, since such \emph{linear vector precoding} can be improved via \emph{non-linear vector precoding} that jointly optimizes precoded vectors $x_{1:M}^1, ..., x_{1:M}^K$ across $K$ channel uses in the aim at improving the \emph{average sum spectral efficiency}, we follow the similar approach as in the previous subsection to apply non-linear vector precoding via
% \begin{align} \label{eq:joint_infty_fronthaul}
%     \tilde{x}_{1:M}^1,...,\tilde{x}_{1:M}^K  &= \arg \min_{ \tilde{x}_{1:M}^1,...,\tilde{x}_{1:M}^K } \sum_{k=1}^K \sum_{n=1}^N \text{EI}_n( [x_m^k]_{m=1}^M ) \nonumber\\&\text{s.t. }{x}_m^k = \sqrt{\frac{K\cdot P_m}{\sum_{k'=1}^K || \tilde{x}_m^{k'} ||^2}} \cdot \tilde{x}_m^k \text{ for all } m=1,...,M,
% \end{align}
% which guarantees the average power constraint
% \begin{align}
% \frac{1}{K}\sum_{k=1}^K || x_m^k ||^2 = P_m.    
% \end{align}
% Solving (\ref{eq:joint_infty_fronthaul}) can be reallized by multiple GD updates. 

% % (\emph{ii}) second \emph{self-normalize} in order to get $(x_m^1)^*,...,(x_m^K)^*$ that satisfy the average power constraint, i.e., $\sum_{k=1}^K || (x_m^k)^* ||^2/K = P_m$, via
% % \begin{align} \label{eq:infty_neural_mq_joint}
% %     {x}_m^k = \sqrt{\frac{K\cdot P_m}{\sum_{k'=1}^K || \tilde{x}_m^{k'}) ||^2}} \cdot \tilde{x}_m^k,
% % \end{align}
% % for all $m=1,...,M$. 










==> Sections/backup_ch_est.tex <==


\subsubsection{Channel Estimation based on DMRS} We consider DMRS configuration type $1$ that can deal with $8$ orthogonal channel estimation, recalling that we have total number of streams $L = N\cdot L_n = 8$. Given the estimated pilot channel obtained via least squares estimate, we then apply MMSE interpolation \cite{hoeher1997two} to obtain channel estimate for the payload data. Channel statistics for MMSE interpolation is obtained by assuming that multipath components are uniformly distributed in time domain within the upper bound of the delay spread \cite{3gpp}, assuming $95\%$ confidence level. Total power across the multipath components are set to $1$ as we consider normalized channel realization for the experiment. 

In Fig.~\ref{fig:pilot_dmrs} below, we show some preliminary results in the presence of channel estimation error. We plot both the sum spectral efficiency as well as the averaged symbol error rate as a function of fronthaul capacity $B^\text{pilot}$ assumed by DMRS pilot symbols. We set $B_m=64$ for PC, while PC and CP assume precoding sharing across $12\cdot 14$ channel uses (1 RB), hence MMSE interpolation is done within this 1 RB. Note that CP does not require additional fronthaul overhead for pilot transmission. For PC, quantization of the pilot symbols are done via neural-PtPQ by noting that the pilot symbols are designed to be orthogonal across different UEs. We can see that neural-MQ still outperforms CP in the presence of channel estimation error. 












\newpage


% \subsection{Exact Gradient Expression}
% In this subsection, we analyze the computational complexity of the proposed gradient-based neural-MQ (\ref{eq:gradient_based_quan}) by explicitly writing down the gradient in terms of basic operations such as matrix multiplication. Let us first denote as $A_k = \text{diag}(A_{1,k},...,A_{M,K})$ and $c_k = [c_{1,k}^\top,...,c_{M,k}^\top]^\top$  the collection of weight matrices and biases vectors from $M$ RUs at the $k$-th (hidden) layer, i.e., $\theta_m = \{A_{m,k}, c_{m,k}\}_{k=1}^K$ and $\theta_{1:M} = \{ A_k, c_k \}_{k=1}^K$, with which  the output of the $k$-th layer $\tilde{x}_{k}$ can be determined as $\tilde{x}_{k} = g_k(A_k \tilde{x}_{k-1} + c_{k})$ given some activation function $g_k(\cdot)$ at layer $k$, with  $\tilde{x}_0 = \sigma_\tau(r_{1:M})$ and $\tilde{x}_K = \hat{x}$. We particularly consider ELU activation for $g_{k}(\cdot)=\color{blue}{..}$ for $k < K$ and identity mapping for $g_K(\cdot)$. Finally, denoting $\text{C2R}(\cdot)$ as a reshaping function that maps a complex vector $\mathbb{C}^{N^\text{tx}}$ to a real vector $\mathbb{R}^{2N^\text{tx}}$ by taking real and imaginary component separately, the gradient in (\ref{eq:gradient_neural_MQ}) can be explicity written as 
% \begin{align} \label{eq:gradient_neural_MQ}
%     &\nabla_{r_{1:M}} \sum_{n=1}^N \text{EI}_n(x, f(\sigma_\tau(r_{1:M})|\theta_{1:M})  ) \nonumber\\&= \text{diag}\bigg( \frac{e^{-r_{1:M}/\tau}}{\tau \cdot (1+ e^{-r_{1:M}/\tau} )^2} \bigg)\cdot \prod_{k=1}^K  A_{k}^\top \text{diag}\Big( \text{ReLU}(A_k \tilde{x}_k + c_k) + \text{ReLU}(-A_k \tilde{x}_k - c_k)e^{A_k \tilde{x}_k + c_k}\Big) \nonumber\\
%     &\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\cdot \text{C2R}\bigg( \sum_{n=1}^N \Big( 2\text{Re}( G_n^\dagger(G_n \tilde{x}_{K} - s_n)  ) \Big) \bigg)
% \end{align}

% which requires computatational complexity ... diagonal... parallel across M ... 


%A_{k}^\top \text{diag}\bigg( \text{ReLU}(A_k \tilde{x}_k + c_k) + \text{ReLU}(-A_k \tilde{x}_k - c_k)e^{}\bigg)

% \begin{align}
%     \label{eq:obj_neural_codebook}
%     \min_{ \{f_m(\cdot)\}_{m=1}^M } \mathbbm{E}\bigg[ \sum_{n=1}^N \text{EI}_n(\hat{x}) \bigg]& \nonumber\\
%     \text{s.t. } (\ref{eq:neural_MQ_overall}),&
% \end{align}






% However, as constrained optimization for neural network is often a challenging task unlike constrained convex optimization problem, we instead train the neural network in an \emph{unconstrained} manner, then to impose the average power constraint in a \emph{post-hoc manner}, which will be specified in the next subsection. Accordingly, training the neural codebook $f_m(\cdot)$ can be simply done by solving
% \begin{align}
%     \label{eq:neural_codebook_opt}
%     &\min_{  \{f_m(\cdot)\}_{m=1}^M  } \mathbbm{E}_{H,s}\bigg[ \sum_{n=1}^N  \text{EI}_n(  f(b_{1:M})  ) \bigg] \nonumber\\
%     &\text{ s.t. }  b_{1:M} = \texttt{neural-MQ}(s, H, W, F|f_1,...,f_M),
% \end{align}
% where the expectation is approximated with available channel realizations and symbol realizations. In the following section, we will show how we impose average power constraint during neural-MQ process hence, to modify the optimization (\ref{eq:neural_codebook_opt}) accordingly.


% \subsection{Achieving Average Power Constraint via Self-Normalization}
% Training the neural codebooks $\{f_m(\cdot)\}_{m=1}^M$  via  (\ref{eq:neural_codebook_opt}) does not guarantee the average power constraint (\ref{eq:avg_power_constraint}). In order to satisfy the condition (\ref{eq:avg_power_constraint}) for each channel realization $H$, we consider \emph{joint optimization} across multiple $K$ channel uses during the channel coherence time, and impose the average power constraint across the $K$ channel uses. To begin with, let us denote $b_{1:M}^k$ as the binary vectors for $M$ RUs obtained by neural-MQ given symbol $s^k$ at channel use $k$. The $K$ binary vectors $ b^1_{1:M},...,b^K_{1:M}$ across $K$ channel uses can be jointly obtained by solving
% \begin{align} \label{eq:N_MQ_obj_joint}
%     b^1_{1:M},...,b^K_{1:M} &= \arg\min_{b^1_{1:M}, ..., b^K_{1:M} }  \sum_{k=1}^K \sum_{n=1}^N \text{EI}_n( [(\hat{x}_1^k)^\top,...,(\hat{x}_M^k)^\top]^\top ),\nonumber\\
%     &\text{ s.t. } \hat{x}_m^k = \sqrt{\frac{K\cdot P_m}{\sum_{k'=1}^K || f_m( b^{k'}_{m}) ||^2}} \cdot f_m(   b^k_{m}    ) \text{ for all } m=1,...,M
% \end{align}
% which can be solved via gradient-based approach as done in (\ref{eq:gradient_based_quan}). Note that in (\ref{eq:N_MQ_obj_joint}),  the transmit vector $\hat{x}^k_m$ for each RU $m$ at channel use $k$ is \emph{self-normalized}, which guarantees the average power constraint across $K$ channel uses, i.e., 
% \begin{align}
% \frac{1}{K}\sum_{k=1}^K || \hat{x}_m^k ||^2 = P_m.    
% \end{align}
% Algorithm~\ref{alg:joint_neural_MQ} summarizes the joint neural-MQ procedure, and we have denoted $[\hat{x}_m]_{m=1}^M$ as $\hat{x}$, i.e., $[\hat{x}_m]_{m=1}^M= [\hat{x}^\top_1,...,\hat{x}^\top_M]^\top$.

% Assuming such joint optimization of neural-MQ, the optimization procedure of neural codebook can be as well modified by taking joint neural-MQ process in Algorithm~\ref{alg:joint_neural_MQ} in lieu of \texttt{neural-MQ}$(s,H,W,F|f_1,...,f_M)$ in (\ref{eq:neural_codebook_opt}). More precisely, denoting  \texttt{neural-MQ}$(s^{1:K},H,W,F|f_1,...,f_M)$ as the algorithmic function that corresponds to Algorithm~\ref{alg:joint_neural_MQ}, the neural codebooks can be optimized by solving
% \begin{align}
%     \label{eq:joint_neural_codebook_opt}
%     &\min_{  \{f_m(\cdot)\}_{m=1}^M  } \mathbbm{E}_{H,s}\bigg[ \sum_{k=1}^K \sum_{n=1}^N  \text{EI}_n\bigg( \bigg[  \sqrt{\frac{K\cdot P_m}{\sum_{k'=1}^K || f_m( b^{k'}_{m}) ||^2}} \cdot f_m(   b^k_{m}    )  \bigg]_{m=1}^M \bigg) \bigg] \nonumber\\
%     &\text{ s.t. }  b^1_{1:M},...,b^K_{1:M} = \texttt{neural-MQ}(s^{1:K}, H, W, F|f_1,...,f_M).
% \end{align}








% \subsection{Infinite Fronthaul Benchmark}

% {\color{blue} Surprisingly, neural-MQ without binary constraint (without temperature anealing to send $\tilde{b}_{1:M}$ directly using infinite fronthaul) was outperformed by neural-MQ. I suspect this is somehow related to generalization analysis but let me figure this out shortly so that we can have proper, tighter, upper bound for our neural-MQ .. }

% Given infinite fronthaul capacity, DU can losslessly transmit the precoded vector $x_m = W_{m,:} s$ to each RU $m$. However, since such \emph{linear vector precoding} can be improved via \emph{non-linear vector precoding} that jointly optimizes precoded vectors $x_{1:M}^1, ..., x_{1:M}^K$ across $K$ channel uses in the aim at improving the \emph{average sum spectral efficiency}, we follow the similar approach as in the previous subsection to apply non-linear vector precoding via
% \begin{align} \label{eq:joint_infty_fronthaul}
%     \tilde{x}_{1:M}^1,...,\tilde{x}_{1:M}^K  &= \arg \min_{ \tilde{x}_{1:M}^1,...,\tilde{x}_{1:M}^K } \sum_{k=1}^K \sum_{n=1}^N \text{EI}_n( [x_m^k]_{m=1}^M ) \nonumber\\&\text{s.t. }{x}_m^k = \sqrt{\frac{K\cdot P_m}{\sum_{k'=1}^K || \tilde{x}_m^{k'} ||^2}} \cdot \tilde{x}_m^k \text{ for all } m=1,...,M,
% \end{align}
% which guarantees the average power constraint
% \begin{align}
% \frac{1}{K}\sum_{k=1}^K || x_m^k ||^2 = P_m.    
% \end{align}
% Solving (\ref{eq:joint_infty_fronthaul}) can be reallized by multiple GD updates. 

% % (\emph{ii}) second \emph{self-normalize} in order to get $(x_m^1)^*,...,(x_m^K)^*$ that satisfy the average power constraint, i.e., $\sum_{k=1}^K || (x_m^k)^* ||^2/K = P_m$, via
% % \begin{align} \label{eq:infty_neural_mq_joint}
% %     {x}_m^k = \sqrt{\frac{K\cdot P_m}{\sum_{k'=1}^K || \tilde{x}_m^{k'}) ||^2}} \cdot \tilde{x}_m^k,
% % \end{align}
% % for all $m=1,...,M$. 









